CoCoFuzzing: Testing Neural Code Models with Coverage-Guided Fuzzing

Deep learning-based code processing models have shown good performance for tasks such as predicting method names, summarizing programs, and comment generation. However, despite the tremendous progress, deep learning models are often prone to adversarial attacks, which can significantly threaten the robustness and generalizability of these models by leading them to misclassification with unexpected inputs. To address the above issue, many deep learning testing approaches have been proposed, however, these approaches mainly focus on testing deep learning applications in the domains of image, audio, and text analysis, etc., which cannot be directly applied to neural models for code due to the unique properties of programs. In this paper, we propose a coverage-based fuzzing framework, CoCoFuzzing, for testing deep learning-based code processing models. In particular, we first propose ten mutation operators to automatically generate valid and semantically preserving source code examples as tests; then we propose a neuron coverage-based approach to guide the generation of tests. We investigate the performance of CoCoFuzzing on three state-of-the-art neural code models, i.e., NeuralCodeSum, CODE2SEQ, and CODE2VEC. Our experiment results demonstrate that CoCoFuzzing can generate valid and semantically preserving source code examples for testing the robustness and generalizability of these models and improve the neuron coverage. Moreover, these tests can be used to improve the performance of the target neural code models through adversarial retraining.

==> Testing Machine Learning based Code Generation Models/figure/dis1.tex <==
\begin{figure}[t!]
\centering
\begin{subfigure}{0.5\textwidth}
\centering
\input{figure/discussion1.tex}
\end{subfigure}\hfill
\vspace{-0.1in}
\caption{\small 
The performance distribution of affected mutation operators.}
\vspace{-0.1in} 
\label{fig:dis1}
\end{figure}

==> Testing Machine Learning based Code Generation Models/figure/discussion2_1.tex <==
\begin{figure}[th!]
\centering
\footnotesize
%\begin{subfigure}{0.45\linewidth}
%\centering
 \scalebox{.5}{\input{figure/pie_1.tex}}
%\end{subfigure}
\caption{\small The distribution of selected mutation operators in {\neuralCodeSum} mutants dataset.}
\label{fig:dis_2_1}
\end{figure}


==> Testing Machine Learning based Code Generation Models/figure/discussion2_2.tex <==
\begin{figure}[th!]
\centering
\footnotesize
%\begin{subfigure}{0.45\linewidth}
%\centering
 \scalebox{.5}{\input{figure/pie_2.tex}}
%\end{subfigure}
\caption{\small The distribution of selected mutation operators  in {\codeseq} mutants dataset.}
\label{fig:dis_2_2}
\end{figure}


==> Testing Machine Learning based Code Generation Models/figure/discussion2_3.tex <==
\begin{figure}[th!]
\centering
\footnotesize
%\begin{subfigure}{0.45\linewidth}
%\centering
 \scalebox{.5}{\input{figure/pie_3.tex}}
%\end{subfigure}
\caption{\small The distribution of selected mutation operators  in {\codevec} mutants dataset.}
\label{fig:dis_2_3}
\end{figure}


==> Testing Machine Learning based Code Generation Models/figure/new_discussion2.tex <==
\begin{figure*}[t!]
\centering
\begin{subfigure}{0.32\linewidth}
\centering
 \scalebox{.6}{\input{figure/pie_1.tex}}
\caption{{\neuralCodeSum}}
\label{pie:d1}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
	\centering
 \scalebox{.6}{\input{figure/pie_2.tex}}
	\caption{{\codeseq}}
\label{pie:d2}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
	\centering
 \scalebox{.6}{\input{figure/pie_3.tex}}
	\caption{{\codevec}}
\label{pie:d3}
\end{subfigure}\hfill
\caption{ 
The distribution of selected mutation operators on the three models.}
\label{fig:new_dis_conbuild}
\end{figure*}

==> Testing Machine Learning based Code Generation Models/figure/overall.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=1\columnwidth]{figure/Overview.pdf}
\caption{The overview of our proposed {\tool}.}
\label{fig:overview}
\end{figure}

==> Testing Machine Learning based Code Generation Models/figure/pie_1.tex <==
\begin{tikzpicture}
\pie[text=pin, color ={black!3, black!10, black!20, black!30, black!40, black!50, 
black!55, black!60, black!65, black!70}]
{9.05/Op1, 8.39/Op2, 4.43/Op3, 
2.82/Op4, 15.79/Op5, 14.83/Op6,
13.97/Op7, 12.73/Op8, 
13.21/Op9, 4.74/Op10}
\end{tikzpicture}


==> Testing Machine Learning based Code Generation Models/figure/rq2_4_5_6.tex <==
\begin{figure*}[t!]
\centering
\begin{subfigure}{0.32\linewidth}
\centering
\includegraphics[width=0.85\textwidth]{figure/NeuralCodeSum_rq2_4.png}
\caption{{\neuralCodeSum}}
\label{fig:rq_2_ncs}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
	\centering
\includegraphics[width=0.85\textwidth]{figure/code2seq_rq2_5.png}
	\caption{{\codeseq}}
\label{fig:rq_2_cs}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
	\centering
\includegraphics[width=0.85\textwidth]{figure/code2vec_rq2_6.png}
	\caption{{\codevec}}
\label{fig:rq_2_nv}
\end{subfigure}\hfill
\vspace{-0.05in}
\caption{ 
Difference in neuron coverage caused by different mutation operators in the three models.}
\label{fig:rq2_4_5_6_plot}
\vspace{-0.1in}
\end{figure*}

==> Testing Machine Learning based Code Generation Models/figure/rq2_4_plot.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figure/NeuralCodeSum_rq2_4.png}
\caption{Difference in neuron coverage caused by different mutation operators in  {\neuralCodeSum}.}
\label{fig:rq2_4_plot}
\end{figure}

==> Testing Machine Learning based Code Generation Models/figure/rq2_5_plot.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figure/code2seq_rq2_5.png}
\caption{Difference in neuron coverage caused by different mutation operators in  {\codeseq}.}
\label{fig:rq2_5_plot}
\end{figure}

==> Testing Machine Learning based Code Generation Models/figure/rq2_6_plot.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figure/code2vec_rq2_6.png}
\caption{ Difference in neuron coverage caused by different mutation operators in {\codevec}.}
\label{fig:rq2_6_plot}
\end{figure}

==> Testing Machine Learning based Code Generation Models/macros.tex <==
\usepackage{soul}
%\usepackage{times}
%\usepackage[T1]{fontenc}
%\usepackage{textcomp}
%\usepackage{mathpazo}
%\usepackage{lmodern}
\usepackage{hyperref}
\usepackage{multirow}
\usepackage{listings}
\usepackage{fancybox}
\usepackage{enumitem}
\usepackage{graphicx}
%\usepackage{paralist}
%\usepackage{framed}
%\usepackage{multicols}
\usepackage{color}
\usepackage{xcolor}
\usepackage{array}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{url}
\usepackage{tikz}
\usepackage{caption}
\usepackage{pgfplots}
\pgfplotsset{compat=1.16}
\usepackage{pgf-pie}
%\usepackage[usenames,dvipsnames]{xcolor}
\usetikzlibrary{pgfplots.statistics,calc}
\usepackage{algorithm}
\usepackage{algorithmic}

\clubpenalty=100000000 %10000
\widowpenalty=10000000 %10000
\brokenpenalty=10000000 %10000

\usepackage{tcolorbox}
\makeatletter
\newcommand{\mybox}[1]{%
	\setbox0=\hbox{#1}%
	\setlength{\@tempdima}{\dimexpr\wd0+13pt}%
	\begin{tcolorbox}[boxrule=0.5pt, colback=white, arc=4pt,
		left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt]
		#1
	\end{tcolorbox}
}

%
\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%

\definecolor{songcolor}{RGB}{191,191,191}
\newcommand{\todoc}[2]{{\textcolor{#1}{\textbf{#2}}}}
% todo commands:
\newcommand{\todored}[1]{\todoc{red}{\textbf{[[#1]]}}}
\newcommand{\todogreen}[1]{\todoc{green}{\textbf{[[#1]]}}}
\newcommand{\todoblue}[1]{\todoc{blue}{\textbf{[[#1]]}}}
\newcommand{\todogray}[1]{\todoc{Gray}{\textbf{[[#1]]}}}
\newcommand{\todoorange}[1]{\todoc{orange}{\textbf{[[#1]]}}}
\newcommand{\todobrown}[1]{\todoc{brown}{\textbf{[[#1]]}}}
\newcommand{\todopurple}[1]{\todoc{purple}{\textbf{[[#1]]}}}
%
%\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%


\newcommand{\todo}[1]{\todored{TODO: #1}}
\newcommand{\song}[1]{\todoorange{Song: #1}}
\newcommand{\moshi}[1]{\todoblue{Moshi: #1}}
\newcommand{\jinqiu}[1]{\todobrown{JinQiu: #1}}
\newcommand{\jie}[1]{\todopurple{Jie: #1}}

% --- for revision
\newcommand{\rev}[1]{\textcolor{purple}{\st{#1}}}
%\newcommand{\rev}[1]{}   
\newcommand{\add}[1]{\textcolor{green}{\textbf{#1}}}
%\newcommand{\add}[1]{{#1}}

\newcommand{\tool}{\texttt{CoCoFuzzing}}
\newcommand{\neuralCodeSum}{{NeuralCodeSum}}
\newcommand{\neuralcodesum}{{NeuralCodeSum}}
\newcommand{\codeseq}{{CODE2SEQ}}
\newcommand{\codevec}{{CODE2VEC}}

%% space in some tables.  BUT have it here, such that you can always renew it
\newcommand{\ts}{$\;$}
\newcommand{\tS}{$\;$}
\newcommand{\tts}{\ \ \ \ \ }
\newcommand{\tss}{\ \ \ $\;$}
\newcommand{\ttts}{$\;$}
\newcommand{\decentHLine}{\noalign{\hrule height 1.04pt}}


==> Testing Machine Learning based Code Generation Models/sec/abstract.tex <==
{Deep learning-based {code processing} models have shown good performance for tasks such as predicting method names, summarizing programs, and comment generation.} %\rev{Automated program summarization is one of the key activities in software analysis, which targets at generating a readable summary that describes the functionality of a program. With the advancement of deep learning and the availability of large-scale open-source repositories, many deep learning-based automatic program summarization approaches have been proposed. }
However, despite the tremendous progress, deep learning models are often prone to adversarial attacks, which can significantly threaten the robustness and generalizability of these models by leading them to misclassification with unexpected inputs. To address the above issue, many deep learning testing approaches have been proposed, however, these approaches mainly focus on testing deep learning applications in the domains of image, audio, and text analysis, etc., which cannot {be directly applied} to {neural models for code} due to the unique properties of programs.

In this paper, we propose a coverage-based fuzzing framework, {\tool}, for testing deep learning-based code {processing} models. 
In particular, we first propose ten mutation operators to automatically generate valid and semantically preserving source code examples as tests; 
then we propose a neuron coverage-based approach to guide the generation of tests. %\jie{only 1,2, maybe first then is better?}
We investigate the performance of {\tool} on three state-of-the-art neural code models, i.e., {\neuralCodeSum}, {\codeseq}, and {\codevec}. 
Our experiment results demonstrate that {\tool} can generate valid and semantically preserving source code examples for testing the robustness and generalizability of these models and improve the neuron coverage.  
Moreover, these tests can be used to improve the performance of the target neural code models through adversarial retraining.

%via synthesizing adversarial examples by mutations, e.g. image adjustment, noise addition, translation, rotation, etc.
%Although most of them have been examined can achieve competitive performance,  the reliability and robustness of these deep learning based models have not been well explored in existing studies

==> Testing Machine Learning based Code Generation Models/sec/algorithm.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[t]
\caption{\small Coverage-Guided Test Generation in {\tool} \label{alg:algorithm0}}
\hrule
	\begin{algorithmic}[1]
		\small
		\vspace{.2cm}
		\REQUIRE %\scriptsize
		Seed programs \textit{S}, 
		Target neural model \textit{NM},\\
		Mutation function $mutate$; \\
		Mutation operators \textit{Ops}\\
		Neuron count cache $NCount$;\\
		Mutate operator set $MO;$ \\
		%Neural Activation function %$neuronActivation;$\\
		Maximum mutation \textit{MAX}; \\
	
		\ENSURE ~\\
		Generated tests $T$;
		\WHILE {$S$ is not empty}
		\STATE $p \longleftarrow S.pop() $
		\STATE $NC_p \longleftarrow neuronActivation(p, NM) $
        \STATE $mutry = 1$
		\WHILE {mutry $<=$ MAX}
		\STATE $mutry = mutry+1$
		\STATE $mutants \longleftarrow null $
		\STATE $bestIdx = -1 $
		\FOR   {$idx=0; idx<size(MO); idx++$} 
		\STATE $Mutant = mutate(O,p)$; 
		\STATE $Mutants.push(Mutant)$; 
		\STATE $NC_{mu}$ = $newNeuronActivation(Mutant,NC_p,NM)$
		\IF  { $size(NC_{mu})>size(NC_{p}) $}
		\STATE $bestIdx = idx$
		\ENDIF
		\ENDFOR
		\IF  { $bestIdx == -1 $}
		\STATE $break$
		\ENDIF
		\STATE $p=Mutants[bestIdx]$
		\STATE $NC_p = newNeuronActivation(p,NC_p,NM) \cup NC_p$
		\STATE T.push($p$) 
		\ENDWHILE
		\ENDWHILE
	\end{algorithmic}
	\hrule
\end{algorithm}


==> Testing Machine Learning based Code Generation Models/sec/algorithm2.tex <==
\renewcommand{\algorithmicrequire}{}
\renewcommand{\algorithmicensure}{}
\begin{algorithm}[t]
\caption{\small Coverage-Guided Test Generation in {\tool} \label{alg:algorithm0}}
\hrule
	\begin{algorithmic}[1]
		\small
		\vspace{.2cm}
		\REQUIRE %\scriptsize
		\textbf{Input:}
		seed programs \textit{S}; 
		target neural code model \textit{NM};\\
		mutation operators \textit{Ops};
		%Mutate operator set $MO;$ \\
		%Neural Activation function %$neuronActivation;$\\
		Maximum number of mutations \textit{MAX}; \\
        \textbf{Variables:} sets of activated neurons $NC_p$, $NC_{curr}$, \textit{bestActivationSet}; \\
		\ENSURE\textbf{Output:}
		 generated tests \textit{T};
		\WHILE {$S$ is not empty}
		\STATE p $\leftarrow$ S.pop()
		\STATE $NC_p$ $\leftarrow$ neuronActivation(p, NM) 
        \STATE numTries = 1
		\WHILE {numTries $<=$ MAX}
		\STATE numTries++
		\STATE bestMutant $\leftarrow$ null 
		\STATE bestActivationSet $\leftarrow$ $\emptyset$
		\STATE bestActivationCount $\leftarrow$ 0
		\FOR   {op in Ops } 
		\STATE currMutant = apply(p, op)
\STATE \small{$NC_{curr}$ $\leftarrow$ newNeurons(currMutant, $NC_p$, NM)}
		\IF  { size($NC_{curr}$) $>$ bestActivationCount }
		\STATE bestActivationCount $\leftarrow$ size($NC_{curr}$)
		\STATE bestActivationSet $\leftarrow$ $NC_{curr}$
		\STATE bestMutant $\leftarrow$ currMutant
		\ENDIF 
		\ENDFOR
		\IF  { bestMutant == null }
		\STATE break
		\ENDIF
		\STATE p $\leftarrow$ bestMutant
		\STATE $NC_p$ $\leftarrow$ bestActivationSet $\cup NC_p$
		\STATE T.push(p) 
		\ENDWHILE
		\ENDWHILE
	\end{algorithmic}
	\hrule
\end{algorithm}

        %\ENSURE ~\\
		% generated tests \textit{T};
		%\WHILE {$S$ is not empty}
		%\STATE p $\longleftarrow$ S.pop()
		%\STATE $NC_p$ $\longleftarrow$ %neuronActivation(p, NM) 
        %\STATE numTries = 1
		%\WHILE {numTries $<=$ MAX}
		%\STATE numTries++
		%\STATE $mutants \longleftarrow null $
		%\STATE $bestIdx = -1 $
		%\FOR   {$idx=0; idx<size(MO); idx++$} 
		%\STATE $Mutant = mutate(O,p)$; 
		%\STATE $Mutants.push(Mutant)$; 
		%\STATE $NC_{mu}$ = %$newNeuronActivation(Mutant,NC_p,NM)$
		%\IF  { $size(NC_{mu})>size(NC_{p}) $}
		%\STATE $bestIdx = idx$
		%\ENDIF
		%\ENDFOR
		%\IF  { $bestIdx == -1 $}
		%\STATE $break$
		%\ENDIF
		%\STATE $p=Mutants[bestIdx]$
		%\STATE $NC_p = newNeuronActivation(p,NC_p,NM) %\cup NC_p$
		%\STATE T.push($p$) 
		%\ENDWHILE
		%\ENDWHILE

==> Testing Machine Learning based Code Generation Models/sec/approach.tex <==
\section{The Approach of \tool}
\label{sec:approach}

%The overall structure of the fuzzing procedure of {\tool} is similar to the structure of coverage-guided fuzzers for deep neural models for image classification, i.e., TensorFuzz~\cite{odena2019tensorfuzz} and Deephunter~\cite{xie2019deephunter}.
%The main differences are: 1) different seed selection strategy and  2) different mutation operators. 
%Specifically, 

%\noindent\textbf{Overview}. 
\input{figure/overall}
In this section, we describe the approach of {\tool}.
Figure~\ref{fig:overview} shows the overview and Algorithm~\ref{alg:algorithm0} describes the main algorithm in detail. 
{\tool} takes a set of initial seed programs and a neural code model as the input, and produces new test sets iteratively through mutation generation (Section~\ref{sec:step1}) and neuron coverage analysis (Section~\ref{sec:step2}).

%{\tool} maintains an operator queue which contains the mutation operators that achieve higher neuron coverage from the last run and generates tests with mutation operators from the queue. 
\subsection{Overview of {\tool}}
\label{sec:overall}
\input{sec/algorithm2}
Algorithm~\ref{alg:algorithm0} shows how {\tool} works step by step.
{\tool} begins by selecting one seed program from
the seed queue (line 1--2), then performs source code transformations to the input based on a list of pre-defined mutation operators (line 11). Given the non-trivial search space constructed by combinations of mutation operators, {\tool} employs a neuron coverage-guided (short for NC-guided) approach (line 5--25), to search for certain types of mutated programs. At a high level, {\tool} searches for program mutations that activate new neurons (line 13--17) while controlling the maximum mutations on one seed program (line 5 and a threshold \textit{MAX}), for both naturalness and the feasibility of utilizing metamorphic testing (i.e., mutated programs can use the same test oracle as the seed program). 
%\jinqiu{I polished the overview, the following two sentences can be moved to neuron coverage analysis} \rev{Each iterator, {\tool} tries all the mutation operators to generate mutants and keeps the one that achieves the maximum new neuron activation.  Then mutated inputs can be fed to the neural network and two things are extracted in {\tool} from the neural network: the activation arrays, which will be used to compute the neuron activation and the output of the neural network, which will be used to evaluate the generated test by comparing to its oracle. }
%{\tool} uses the new neuron activation between the original seed program and its generated mutants to maintains the generated test set, i.e., mutants with higher neuron activation will be added into the seed program queue. 
%Once a seed program from the queue was chose to mutate, the mutations need to be applied. Lines 2 to 17 in the Algorithm~\ref{alg:algorithm0} shows the details of the mutation generation process, which takes a seed program $p$ and the maximum mutation try $L$ as input to create a set of newly generated tests $T$ as the output. To generate a test, {\tool} exhausts the ten mutation operators and keeps the one that achieves the maximum neuron coverage. 

% \jie{Does `creating test oracles' need to be in Figure 1.} \song{modified}
% \jie{This is corresponding to the `neuron coverage analysis' in Figure 1? Maybe should state it more clearly, otherwise, the readers might do not find the related subsections for this box.}
% \jie{The subsection C is `generating test oracles', can we rename the title or Figure 1 to let them align with each other? Because `Oracle' in figure 1 can be renamed and use a different icon as `mutation generation'?}
% \jie{Overall, i see Figure 1 is not very aligned with the descriptions. May need to revise it.}

%Existing fuzzers for classic deep learning applications (e.g., image)~\cite{odena2019tensorfuzz,tian2018deeptest,xie2019deephunter} use the metamorphic relations between seed images and the generated test images via transformation to infer the oracles~\cite{chen2020metamorphic}. 
%Specifically, they generate new test images through predefined transformation operators with the intention that a new test image and its original seed image should share the same semantics from a human perspective and adding a little perturbation to the seed image would not change the human decision, so if a deep neural network is unable to correctly recognize the image after transformation, it reveals a defect in the deep neural network. 
%Different from them, we directly use the ground-truth of an initial seed program as the oracle of all the test cases derived from it since all the used ten types of program transformation do not change the semantic of the program.

%\todo{Moshi: description of the algorithm}

Note that in traditional coverage-guided fuzzers for computer programs~\cite{serebryanylibfuzzer,zalewski2014american}, a seed can be reused and mutated for multiple times, e.g., these tools often use either time constraints or the number of generated mutants as the termination condition and a single seed can generate thousands of mutants~\cite{rebert2014optimizing}. 
However, a similar process cannot be directly applied for testing neural code models as there are no explicit oracles (i.e., program crashes) available to assess the result of a seed program mutated multiple times~\cite{xie2019deephunter}. To bypass the oracle challenge in testing neural code models, we leverage metamorphic testing, similar to \cite{xie2019deephunter,tian2018deeptest}. A mutated program shares the same oracle as the seed program if the transformation is semantic-preserving. 
Note that mutating a program could hurt its naturalness as the inserted/mutated code could be noise to the original program.  
Hence, we use a threshold $MAX$ to limit the maximum number of mutations applied on a seed program, which means a seed program at most can be mutated for $MAX$ times accumulatively. 
{Note that the design of $MAX$ controller does not guarantee the naturalness of the inserted mutation code. A robust code model should have the ability of ignoring the inserted noise code despite its naturalness.} % and to ensure the generated mutants preserve the same semantics as the original seed program {while maintain a certain level of naturalness.}  
%For all the subsequent experiments in this paper, 
%\add{to find an appropriate value for $MAX$, we }
%we limit the maximum mutations to three, which means a seed program at most can be mutated for three times accumulatively (details in Section~\ref{sec:max}\jinqiu{Consider moving  the discussion here}. 
%\moshi{do we have enough explanation to the naturalness?}
%\input{sec/algorithm}

%\subsection{Setting of Threshold $MAX$}
%\label{sec:max}
%{\tool} uses a threshold $MAX$ to limit the maximum number of mutation tries on a seed program as inserting too many mutants into a seed program could dramatically hurt its naturalness. %as the inserted code could be noise to the original program.  
To find an appropriate value for $MAX$, we randomly selected 1,000 sample programs from the test datasets of the three studied neural code models (details are in Section~\ref{sec:sub}). For each sample, we randomly select $MAX$ mutation operators and apply them to the given sample to generate mutants.  
We experiment $MAX$ with values from 1 to 10. 
{In the most conservtive senario, we assume the generated code are entirely un-natural}.Hence, We measure the naturalness of the mutated program by using the percentage of the generated code.

\input{figure/dis_max}
%\todo{moshi: update the figure}
Figure~\ref{fig:dis_max} shows the average percentage of generated code against the seed program under different $MAX$. 
With the increass of $MAX$, the naturalness of code decreases dramatically. For example, when $MAX$ is equal to 1, on average only 9.25\% code in a mutated program is noise (i.e., generated code), while $MAX$ increases to 10, the percentage of noise code is 59.60\% on average. 

Prior work showed that overall there is about 28\% noise code in real-world software projects~\cite{eder2012much}. %To simulate the statistics of real-world software,} 
Thus, for all the subsequent experiments in this paper, 
%\add{to find an appropriate value for $MAX$, we }
we set $MAX$ to three, which yields less 30\% noise code on average. 
%means a seed program at most can be mutated for three times accumulatively.


\begin{comment}
\subsection{Seed Program Selection}
\label{sec:step0} 
\song{Remove this subsection}
Seed selection decides which seed should be picked next to generate new test via mutation. 
%Traditional fuzzers~\cite{serebryanylibfuzzer,zalewski2014american} often use executable code coverage as a seed selection strategy and prefer to choose the seed that covers more code path in the seed queue. Motivated by this, 
The current fuzzing techniques for deep neural networks~\cite{odena2019tensorfuzz,tian2018deeptest} adopted a uniform sampling strategy that randomly
selects a seed from the seed queue to generate mutants. 
%follow the similar idea to prioritize selection of seed based on the neuron coverage.  
Recently DeepHunter~\cite{xie2019deephunter} proposed to use the number of times a seed has been fuzzed as the strategy to select seeds and give a higher probability to seeds that have been mutated fewer times. Experiment results showed their strategy can outperform the random selection.  
In this work, we use the uniform sampling strategy rather than DeepHunter's strategy for the following reason. 
Current fuzzing techniques for deep neural networks~\cite{odena2019tensorfuzz,tian2018deeptest,xie2019deephunter} mainly focus on image classification models. Given a seed image,
there is no limitation for the number of tests generated from it. 
Thus, it's possible that a large number of tests are generated from the same images, which will hurt the effectiveness and diversity of the fuzzers. 
DeepHunter used the number of times a seed has been fuzzed to balance the diversity and recency of seed selection.
While the above issue does not exist in {\tool}, as it uses a threshold $MAX$ to limit the maximum number of mutations tries on a seed program and to ensure the generated mutants preserve the same semantics as the original seed project.
In this work, we set $MAX$ to three, which means a seed program at most can be mutated for three times. 

Thus, in each iteration of {\tool}, 
the last seed is picked from the seed queue, and new tests are generated based on it. The generated new test is added to the seed queue if it improves the neuron coverage. 
For a selected seed, if all of the generated tests cannot improve the coverage or the number of mutations applied on it is equal or larger than 3, the seed and its generated tests will be removed from the queue. 
\end{comment}
\subsection{Neuron Coverage Analysis}
\label{sec:step2}
%\todo{Moshi: explain these methods in the algorithms}
Algorithm~\ref{alg:algorithm0} details how {\tool} uses neuron coverage in searching for new test data (line 5--25). In each iteration (line 10--18), {\tool} tries all the mutation operators and identifies one mutated program that activates the most number of new neurons. This mutated program is produced as one test data (line 24) and also kept for the next mutation iteration. Controlled by the threshold \textit{MAX} (line 5), this mutant might be continuously mutated in the next iteration, until the number of mutations applied per original seed program reaches the threshold, which is empirically set to three in our experiments.
%Then mutated inputs can be fed to the neural network and two things are extracted in {\tool} from the neural network: the activation arrays, which will be used to compute the neuron activation and the output of the neural network, which will be used to evaluate the generated test by comparing to its oracle.

Two methods \textit{neuronActivation} and \textit{newNeurons} in Algorithm~\ref{alg:algorithm0} are for neuron coverage analysis. 
The \textit{neuronActivation} method takes a trained neural model and one input and produces a set of activated neurons as output. {For example, given a trained model in {PyTorch}}, we inject listeners to monitor the neurons. 
Then, we run the inference or prediction of the trained model with the input and collected the output of each neurons using the injected listeners. 
Similar to prior work~\cite{tian2018deeptest,xie2019deephunter}, for each neuron, we scale the value of the neuron to the range of 0 to 1 and compare the scaled value to a threshold. 
If the scaled output is greater than the threshold (i.e., we use 0.4, the same value with \cite{tian2018deeptest,xie2019deephunter}), we consider the neuron activated, otherwise inactivated. 

%Finally, we collected all activated neurons labeled with the layer name concatenated with its index as the output of method \textit{neuronActivation}. 
The \textit{newNeurons} method is very similar to \textit{neuronActivation}, which takes a model, one input data, and a set of activated neurons (i.e., $NC_p$ in line 12) as the input. The method \textit{newNeurons} calculates the activated neurons by the input, and outputs a set of newly activated neurons by the input but not $NC_p$. %\textit{neuronActivation} is that \textit{newNeurons} substracts a set of neurons $NC_p$ from the activated neurons by the input.
%The output of the \textit{newNeurons} is additional activated neurons compared to $NC_p$.
The implementation of neuron coverage analysis in {\tool} is model-independent and can be widely applied to various deep learning models.

\subsection{Mutation Generation}
\label{sec:step1}
In \tool, we adopt and implement specialized mutation operators for mutating programs. To bypass the oracle problem, our proposed mutation operators preserve program semantics. Hence, the mutated programs should have the same test oracles with the original programs, i.e., metamorphic testing.
Prior studies~\cite{tian2018deeptest, xie2019deephunter} in testing neural models propose mutation operators for inputs such as image and audio, e.g., image scaling, image rotation, and noise addition, etc. These operators cannot be directly applied to source code programs as programs must strictly follow the rigid lexical, grammatical, and syntactical constraints. %Also the mutated programs are expected to fully preserve the original program semantics.

In this work, we propose to use a set of ten mutation operators that can be applied to method level to generate
semantically-equivalent methods. The mutation operations include transformations
ranging from common refactoring like variable renaming to more intrusive ones like adding unreachable branches. Table~\ref{tab:opts} summarizes the ten mutation operators and how each mutation operator can be applied to transform a program. 
Note that, among the ten operators, \textit{Op1} and \textit{Op10} are proposed and experimented  in prior  studies~\cite{yefet2019adversarial,zhang2020generating} to generate adversarial examples for neural code models. The other eight mutation operators are first used in this work. These mutation operators target at a diverse types of program transformations.
%~\jinqiu{how these mutation ops are implemented?}
%\todo{moshi: give high-level description here}

We use the open-source java parser package javalang\footnote{\url{https://pypi.org/project/javalang/}} 
for code parsing and tokenization. 
Given a program $T$ and a mutation operator $O$, %we first parse the code and identify all the available positions for mutation regards to operator $O$. 
we first use the AST parser from javalang to convert $T$ to a list of sub-AST where each element is the AST representation of a statement. 
We then iterate the sub-AST list and mark the possible positions for $O$ regarding its specific transformation requirements. The detailed process of mutation generation for each operator is as follows.


%We then split $T$ to statement level using the sub-AST list and mark the location between statements as available position for injection.
%Then we apply $O$ into one of the available . Note that some operators has only one available injection location. 
%We verify the mutants by using javalang again and collect only the successful mutants.
%\song{Theoretically all mutants should be successful} 

%\jinqiu{Consider removing the following sentence as it may get readers confused about the approach, in the end these are still individual ops} 
%We group some options that share the same procedure together, e.g., \textit{Op5} to \textit{Op9} add unreachable branches by using different types of control flow structures. 

\begin{itemize}
\item \textbf{(Op1) Dead store~\cite{yefet2019adversarial}:} inserts an unused variable declaration with one primitive type (e.g., string, int, double, and long, etc.) to a randomly selected basic block in the program.  %\jinqiu{method to program, change it throughout the paper}
The name of the variable is a string of eight characters randomly generated in the form of [a-z]. %~\jinqiu{is 8 supported somehow? any references or similar prior work?} 
Only one dead store is added in each transformation by this operator.

\item \textbf{(Op2 and Op3) Obfuscating:} rewrites a numerical value or variable and its usages in a statement by adding and deleting the same random numerical value of the same type. For example, $x = 1.0;$ can be mutated to ${x = 1.0 + 0.1 -0.1;}$ or $x = 1.0+0-0;$. If one program contains more than one numerical variables, we randomly pick one to perform the transformation. This operator only works on assignment, declaration, or return statements.

\item \textbf{(Op4) Duplication:} duplicates a randomly selected assignment statement and insert immediately after its current location. To avoid side-effect, the applicable assignment statement is limited to the ones without using method invocation.%to avoid changing the semantic of the program. 

\item \textbf{(Op5 to Op9) Unreachable loops/branches:} inserts an unreachable loop or branch (including \textit{if} statement, \textit{for} statement, \textit{while} statement, and \textit{switch} statement) into a randomly selected basic block in the program. 
The condition of the inserted loop or branch is always false to make it unreachable. 
%\rev{For simplifying our implementation, we insert a dead store in the body of an unreachable loop/branch.}%\moshi{No, not empty. Updated, pls review } 

\item \textbf{(Op10) Renaming~\cite{yefet2019adversarial,zhang2020generating}:} renames a local variable declared in a program. If there exist multiple variables, we randomly select one for the mutation. The new name of the variable will be in the form of [a-z]. %~\jinqiu{also 8, great if we can use any references.}
%\jinqiu{Is ours exactly the same with the two references? Op1 and Opt10 can use a bit more description on that.}\song{They did not give description, directly showed in code examples}
\end{itemize}

\input{table/mutationOpts}
%\subsubsection{Neuron Coverage Guided Operator Selection}
%\label{sec:step2} 

%\jinqiu{The following paragraph can be merged with algorithm design}

Note that some of the proposed operators, i.e., \textit{Op1} and \textit{Op5}--\textit{Op9}, can be inserted into any locations in a given program. In this work we randomly pick a location to apply these mutation operators because through experiments we find that the chosen locations are not correlated with the effectiveness of these mutation operators (details are in Section~\ref{sec:dis1}). 


%\subsection{Creating Test Oracles}
%\label{sec:step2}
%\rev{Traditional fuzzers~{serebryanylibfuzzer,zalewski2014american} mutate a seed with bytewise flips, block/statement replacement, and input file modifications, etc. These mutants do not have the oracles issues as they are evaluated via whether or not they can cause abnormal behaviors of the system under test, e.g., system crash. However, abnormal behavior of a deep neural network is the disagreement between the output of neural networks and a human decision. To address this issue, }
 
% \jie{
% Not sure whether we need this long introduction, which is like the background. Maybe we can reduce them to 1-2 sentence?}

%Inspired by the existing fuzzers for deep neural networks~\cite{odena2019tensorfuzz,tian2018deeptest,xie2019deephunter}, 

%we used the data set from Code2Seq for our experiments in Code2Seq and Code2Vec. There are three dataset provided by code2seq which are java-large with  417003 testing examples; java-med with 
%odena2019tensorfuzz,tian2018deeptest} adopted a uniform sampling strategy that randomlyselects a seed from the seed queue to generate mutants. 
%follow the similar idea to prioritize selection of seed based on the neuron coverage.  Recently DeepHunter~\cite{xie2019deephunter}

%we created a python-based java code mutation library using the javalang python package. the library takes a pice of java method and run through a list of mucation options to generate an mutated java method. the mutation is sementic-preserved. that means the meaning ande the result of the given java method is invariant before and after the mutation.

==> Testing Machine Learning based Code Generation Models/sec/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
This work proposes a coverage-based fuzzing framework, {\tool}, for testing deep learning-based models for code processing. In particular, we first propose and implement ten mutation operators to automatically generate valid (i.e., semantically preserving) source code examples as tests; 
we then propose a neuron coverage-based approach to guide the generation of tests.  
We investigate the performance of {\tool} on three state-of-the-art and typical neural code models,  i.e., {\neuralCodeSum}, {\codeseq}, and {\codevec}.  Our experiment results demonstrate that {\tool} can generate diverse and valid tests for examining the robustness and generalizability of neural code models. 
Moreover, the generated tests can be used to improve the performance of the target neural code models through adversarial retraining. 

==> Testing Machine Learning based Code Generation Models/sec/discussion.tex <==
\section{Discussions}



\label{sec:discussion}

% \jie{Do we need to say something about the potential effectiveness of this proposed method compared with the variable renaming and others? Because we donot treat them as baselines, it might be argued. }
% \song{added in RQ2}
%\todo{Moshi r1 random *10}

% \subsection{The naturalness of code model}
% \label{sec:natualness}
%  \song{you always use "works", work is uncountable}
%  {There exist many studies~\cite{hindle2012naturalness,raychev2014code,alon2019code2vec} \song{multi citation always put into one cite command} \song{ use a ~ between cite and context before} that apply language model approach to code in recent years.
%  These studies show that programming languages have many similar characteristics compare to natural languages\cite{hindle2012naturalness}. Many code models depend\rev{s} on the naturalness of the code and are build on top of the belief that the training programs collected from existing projects are the natural representation of the programming language~\cite{raychev2014code,gu2016deep}. However, unlike language model, Naturalness may not be meaningful to code model because the semantic of software programs is define by compiler and test-cases\cite{ammann2016introduction}. A program could become less natural and also semantic-preserve by replacing the variables to hash code. Our experiment shows that the code model performance is reduced significantly and thus not robust if the naturalness of the code reduces with basic attack patterns. Note that instead of exploit the naturalness, we limit the naturalness reduction by limiting the percentage of generated code within the general percentage of unused code for natural software programs to better simulate the real-world programs \cite{eder2012much}. 
%  \mybox{\add{Our results show that the dependency to naturalness of the programs makes the code model vulnerable to neural-coverage guided attack. The performance of code models reduce significantly if the naturalness assumption do not hold.}}
% }

\subsection{Impact of the Applied Locations of Mutation Operators}
\label{sec:dis1}
Some of the mutation operators in {\tool} can be applied in any locations in a given program (i.e., location independent). For example, \textit{Op1} inserts an unused variable declaration into a randomly selected basic block of in a program, thus for any non-empty program there exists more than one location for \textit{Op1}. 
Among the ten mutation operators listed in Table~\ref{tab:opts}, \textit{Op1} and  \textit{Op5}--\textit{Op9} are location independent. 
To better understand the impact of this randomness on the performance of \tool, for each location independent operator, we apply it on the \textit{1K  original} test dataset to get a new test dataset. Then we collect the performance of the three models on the new test datasets. We rerun the above process 10 times and calculate the standard deviation values and the distribution of the performance of the three neural models. Table~\ref{tab:ds_1} shows the detailed results.  

We find that, for all the location-independent operators, their effectiveness on neural code model is insensitive to the applied locations, i.e., the variance is small. 
%We further conduct One-Way ANOVA test on the performance set of each model on each operator, the 
Our One-Way ANOVA test results show that there is no significant difference among the performance of the 10 runs, which suggests that the locations of generated mutants do not significantly impact the effectiveness of {\tool}. Thus, in our experiments we randomly pick a location to apply these mutation operators.
 %\mybox{\add{Our One-Way ANOVA test results suggests that the locations of generated mutants do not significantly impact the effectiveness of {\tool}.}}
%Thus, in this work, for each of the 
\input{table/ds_1}
\subsection{Distribution of the Selected Mutation Operators}
\label{sec:dist}
%\input{figure/discussion2_1}
%\input{figure/discussion2_2}
%\input{figure/discussion2_3}
%\input{figure/new_discussion2}
\input{table/ds_2}
%Figure~\ref{fig:new_dis_conbuild}

{\tool} adopts a neuron coverage guidance algorithm to generate new tests with the ten pre-defined mutation operators. 
To further understand the operator selection process in {\tool}, we collected the selected operator for each mutant generated by {\tool} for each of the three neural code models, i.e., {\neuralCodeSum}, {\codeseq}, and {\codevec}. 
Table~\ref{tab:ds_2} shows the percentage of each operator used among the tests generated by {\tool} on each model. 
Overall, we can see that distribution of the selected operators varies dramatically among different neural code models, e.g., \textit{Op10} was used among 5\% of all the generated tests in {\neuralCodeSum} while less than 1\% of the generated tests from {\codeseq} used \textit{Op10}. 
In addition, we can also see that some of the operators are dominating across different models e.g, \textit{Op5} has been used in more than 15\% of the generated tests on each model. While these also exist {in the} operators that are selected less frequent across the three models, i.e., \textit{Op1},\textit{Op3}, \textit{Op4}, and \textit{Op10} are used in less than 10\% of the generated test cases across the three models. 
{One of the possible reasons is that \textit{Op5} activates relatively more new neurons than other operators (As shown in Table~\ref{tab:rq2_nc}). 
We have conducted Spearman rank correlation to compute the correlation between the number of newly activated neurons of mutants generated by an operator and the frequency of an operator used in a neural code model. The Spearman correlation values are 0.78 in {\neuralCodeSum}, 0.68 in {\codeseq}, and 0.92 in {\codevec}, which indicates that the frequency of an operator used in a neuron code model is positively correlated with its ability to activate new neurons (compared to the original tests).}
% \jie{Do we need to refer to the relative contribution of each operator in Table IV to better illustrate their role? }
%While these also exist {in the} operators that are selected less frequent across the three models, i.e., \textit{Op1}--\textit{Op4} and \textit{Op10} are used in less than 10\% of the generated test cases across the three models. 
%The main reason for this is that tests generated by them have less impact on affecting the performance of the examined code models than other operators as shown in RQ1 (Section~\ref{sec:rq1}). 
%Figure~\ref{pie:d2} shows very similar result to Figure~\ref{pie:d1}. Over 75\% of the selected operators in {\codeseq} mutants dataset are from \textbf{Op5} to \textbf{Op9}, which are the operators that have strong impact against {\codeseq}.  Figure~\ref{pie:d3} shows similar result to Figure~\ref{pie:d2}. 
%Note that the three models are designed for different deep learning tasks, so there are differences in the percentages of operator 5 to 9 across three models. e.g. operator 5 takes 15.8\% of the distribution in {\neuralCodeSum}, 19.2\% in {\codeseq} and 26.0\% in {\codevec}. 
%\mybox{\add{Overall, mutation operators with a stronger impact on the performance of a neural code model are selected more often by {\tool} than other mutation operators. }}

%Given the fact that we compare all the options and select the most effective operator in each mutation step of NC-guided algorithm, the selected operators are distributed in all classes instead of just one class.
\subsection{Threats to Validity}
\label{sec:threats}
The selection of the studied neural code models and experimental projects could be a threat to validity. 
In this work, we only evaluated {\tool} on {\neuralCodeSum}, {\codeseq}, and {\codevec} with Java programs. 
Therefore, our results may not generalize to other neural code models or other programming languages. 
We leave the evaluation of the general applicability of our approach as future work. 
To generate new tests, this paper adopts ten different mutation operators for program transformations. 
Although these mutation operators have been examined can help generate effective mutants, these mutation operators may not represent many possible transformations for software programs. 
In addition, most of the used mutation operators are designed for object oriented programming languages, e.g., Java, which might not work for other program languages.
We will extend our approach with more mutation operators for supporting more program languages.  
{\tool} uses a threshold $MAX$ to limit the maximum number of mutation tries on a seed program. We set $MAX$ to three in this work {to simulate the natural statistics of unused code in software projects}, while the performance of {\tool} could vary with different values of $MAX$. We plan to explore the effectiveness of {\tool} with more $MAX$ values in the future. 
In this work, following existing studies~\cite{tian2018deeptest,xie2019deephunter} we use neuron coverage to guide the generation of valid mutants.  
% {Recent studies on neuron coverage suggest that the optimization of neuron coverage sacrifice the naturalness of the model~\cite{li2019structural, dong2019there, harel2020neuron}. However, this is not a limitation to our study as the naturalness of the inserted code should not effect the interpretation of a program if the code model learns the semantic of programs rather than the distribution of token sequences of programs.}


%Traditional fuzzers adopted code coverage to guide the test generation, similarly 
In this work, following existing fuzzers for testing deep learning models, we also use neuron coverage to guide the generation of tests. Although there have been increasing discussions on whether neuron coverage is a meaningful metric, our experiments show that it works for testing neural code models. We plan to examine the effectiveness of {\tool} with more criteria. 
%similar to the discussion on code coverage metrics, despite their unstable correlation with test suite effectiveness, they have been widely applied in fuzzing techniques to guide the search.

==> Testing Machine Learning based Code Generation Models/sec/introduction.tex <==
\section{Introduction}
\label{sec:intro}

%Automated program summarization generates a readable natural language description for a program, which can assist developers to understand program and reduce documentation workload~\cite{allamanis2016convolutional,haiduc2010supporting}. 
%\jinqiu{Understanding program semantics and associating them with natural language descriptions are important tasks in software development. Automated realizations of these tasks lead to many helpful applications, such as comment and commit message generation, to reduce workloads and assist developers in development process~\cite{allamanis2016convolutional,haiduc2010supporting}} Recently, with the advancement of deep learning and the availability of large-scale open-source repositories, many deep learning based automatic program summarization approaches have been proposed~\cite{alon2018code2seq,alon2019code2vec,ahmad2020transformer,iyer2016summarizing,liang2018automatic,hu2018deep,leclair2020improved,allamanis2016convolutional} and most of them have reported spectacular performance on summarizing programs.  
Deep learning (DL) has recently been successfully applied to accelerate many tasks in automated source code processing %\jie{processing? not sure whether we should use process or processing; there are several places for that.},  
such as prediction of variable names~\cite{alon2018code2seq,alon2019code2vec}, code summarization~\cite{ahmad2020transformer,hu2018deep,liang2018automatic,allamanis2016convolutional}, and comment generation~\cite{hu2020deep,chen2019neural}. %code generation~\cite{gu2016deep,brockschmidt2018generative}, and code search~\cite{gu2018deep,cambronero2019deep}. \jie{here we should only consider the case which use source code as input, but code generation and search is using natural language as input? So we should not include them?} 
Most of these deep learning-based code models (i.e., neural code models for short) have reported good performance.  

% \jie{Can we start with all the source code related deep learning approaches (rather than program summarization, which is a quite small area), e.g., code search, comment generation, etc. Because this mutation-based method can used to test all the code-related deep learning approaches theoretically. And in the third para, i also see the examples for the general code-related deep learning approaches. 
% I think we can introduce program summarization in the four para to use it as a case study or something like that. 
% By beginning with a bigger area, this work might look more influential and generalized.}

However, deep learning models are widely known to suffer from adversarial attacks~\cite{ma2018deepgauge,pei2017deepxplore}, i.e., a subtly-modified input can lead neural networks to misclassifications and result in severe erroneous behavior of DL %\jie{should add abbreviation for DL before} 
models. 
%where such input is called adversarial example and the process to generate adversarial examples is known as adversarial attack~\cite{madry2017towards}. Adversarial examples can be generated from original inputs by carefully designed minor perturbations, which have little or no difference from their original counterparts by human perceptions. 
More thorough testing of neural networks can improve their reliability and robustness. %against adversarial examples, 
Many deep learning testing approaches have been proposed~\cite{xie2019deephunter,tian2018deeptest,zhang2019cagfuzz,alzantot2018generating}, however, most of {these} %\rev{existing deep learning testing} 
approaches mainly focus on generating tests for deep learning models in the domains of image, audio, and text analysis by using mutations such as image adjustment, image scaling, image rotation, and noise addition, etc., which cannot be directly applied to {neural code models}. 
In addition, different from adversarial example generation for image, audio, and natural languages, the structured nature of programming languages brings new challenges, i.e., program must strictly follow the rigid lexical, grammatical and syntactical constraints, and tests generated for a program are expected to fully preserve the original program semantics. 
%semantically equivalent


Recently, some adversarial example generation approaches for source code were proposed, e.g., \cite{zhang2020generating} performed variable name replacements to perturb the programs and \cite{yefet2019adversarial} proposed to use both variables renaming and dead code (i.e., unused variable declaration) insertion to generate semantically equivalent adversarial examples. {However, the types of perturbations introduced by the two transformations are limited, as we have witnessed many other types of noise/perturbation in real-world software programs that sharing the same semantics~\cite{allamanis2019adverse}.  Hence only using the two operators may miss numerous corner cases for the purpose of thoroughly testing neural code models.}
%However, 
%in real-world software programs, there are many other semantic preserving transformations~\cite{allamanis2019adverse}, e.g., add code duplication, add or delete unreachable code, statement refactoring, etc., therefore
%the existing adversarial example generation approaches for testing neural code models can miss numerous corner cases since they only leverage two basic program transformations, i.e., variable renaming and dead code insertion, to generate adversarial examples.
%\jinqiu{However, such transformations are limited compared to nuances in real-world programs and may miss numerous corner cases for the purpose of thoroughly testing neural code models.}

% There are clearly many other semantic preserving transformations (e.g., re-ordering independent statements), but their application would require a deeper analysis of the program to guarantee that they are indeed semantic preserving. 

In this paper, we propose a coverage-based fuzzing framework, {\tool}, to test neural code models.  
Specifically, we first propose and implement ten mutation operators, which represent various real-world semantic preserving transformations of programs, to automatically generate valid and semantically preserving source code examples as tests.  
Then we utilize a neuron coverage based
guidance mechanism for systemically exploring
different types of program transformations and {guiding} the generation of tests. 
We investigate the performance of {\tool} on three state-of-the-art typical neural code models, i.e., {\neuralCodeSum}~\cite{ahmad2020transformer} (leverages a self-attention-based neural network to generate summarization of programs), {\codeseq}~\cite{alon2018code2seq} (builds a AST-based RNN neural network to predict method names), and {\codevec}~\cite{alon2019code2vec} (uses a path-based attention model for learning code embeddings to represent a method).  
%\jie{May need to better summarize the key idea of these three methods. in current version, cannot get a clear understanding of their difference, e.g., the first is self-attention based, the third is attention-based.}\song{revised}
%\jie{Does code2seq also base on path-based? AST-based? since its performance is good}

Our experiment results demonstrate that {\tool} can generate valid and semantically preserving tests for examining the robustness and generalizability of neural code models. Specifically, the newly-generated tests by {\tool} can reduce the performance of {\neuralCodeSum}, {\codeseq}, and {\codevec} by 84.81\%, 22.06\%, and 27.58\% respectively. 
Moreover, we find that these new tests by {\tool} can also be used to improve the performance of the target neural code models through adversarial retraining. 
Specifically, performance can be improved 35.15\% on {\neuralCodeSum}, 8.83\% on {\codeseq}, and 34.14\% on {\codevec} by retraining the models with synthetic data generated by {\tool}. 

This paper makes the following contributions:
\begin{itemize}
\item We propose a coverage-based fuzzing framework {\tool} for testing the robustness of neural code models. 
To the best of our knowledge, {\tool} is the first fuzzing framework for testing neural code models. We have released the implementation of our tool to facilitate the replication of this  study\footnote{https://doi.org/10.5281/zenodo.4000441}.

\item We implement ten mutation operators, which represent various real-world semantic preserving transformations of programs, to automatically generate tests. 

\item We utilize and experiment a neuron coverage-based guidance mechanism for systemically exploring the large search space constituted of different types of program transformations and measure the adequacy of the fuzzing. 
%\jinqiu{Need to discuss and highlight the difference in algorithm, compared to DeepHunter and DeepTest, in later sections}.

\item We evaluate {\tool} on three state-of-the-art neural code process models, i.e., {\neuralCodeSum}, {\codeseq}, and {\codevec}. The experiment results show the effectiveness of our tool. 

\end{itemize}	 
The rest of this paper is organized as follows. 
Section~\ref{sec:bg} presents
the background of neural code models.   
Section~\ref{sec:approach} describes the
methodology of our proposed {\tool}. 
Section~\ref{sec:experiment} shows the setup of our experiments. 
Section~\ref{sec:result} presents the result of our study.  Section~\ref{sec:discussion} discusses the threats to the validity of this work. Section~\ref{sec:related} presents related studies. Section~\ref{sec:conclusion} concludes this paper.

%\todo{song global fix: method -> program}

==> Testing Machine Learning based Code Generation Models/sec/motivation.tex <==

\section{Background}
\label{sec:bg}

\subsection{Neural Code Models}
\label{sec:bg1}
The growing availability of open-source repositories creates new opportunities for using deep learning to accelerate code processing tasks 
%Most of the existing neural program summarization approaches frame the problem as a sequence generation task, i.e.,  both the code and
%the summary is a sequence of tokens that are represented by a sequence of vectors~\cite{shido2019automatic,alon2018code2seq,alon2019code2vec,ahmad2020transformer,iyer2016summarizing,liang2018automatic,hu2018deep,leclair2020improved}. Specifically, they take a method body as their raw input and utilize structural information of a program in the form of Abstract Syntax Tree (AST) as the input to the neural based models, the output is a summary that describes the functionality of the method. 
such as prediction of variable names~\cite{alon2018code2seq,alon2019code2vec,alon2018general}, code summarization~\cite{ahmad2020transformer,hu2018deep,liang2018automatic,allamanis2016convolutional}, and comment generation~\cite{hu2020deep,chen2019neural}.
The deep neural networks used in neural code processing models mainly can be categorized into two types: (1) Recurrent Neural Network (RNN) and (2) Attention Neural Network. 
We provide a brief description of each architecture below.
%and use recurrent encoderdecoder networks with attention mechanisms as the fundamental building blocks.

\noindent \textbf{RNN architecture.}
A recurrent neural network is a neural network that consists of a hidden state $h$ and an optional output $y$ which operates on a variable-length sequence $x=(x_{1}, ... , x_{T})$. And at each time step $t$, the hidden state $h_{t}$ of the RNN is updated
by $h_{t}=f(h_{t-1}, x_{t})$. $f$ is a non-linear activation function. Standard RNNs are not capable of learning ``long-term dependencies'', i.e., they may not propagate information that appeared earlier in the input sequence later because of the vanishing and exploding gradient problems. 
Long short-term memory LSTM~\cite{hochreiter1997long} has been proposed to address the above issue. It introduces additional internal states, called memory cells, that do not suffer from the vanishing gradients and it controls what information will be propagated. 
%Many neural program summarization models~\cite{shido2019automatic,alon2018code2seq,iyer2016summarizing} are built on RNN networks.

\noindent \textbf{Attention network architecture.}
Attention neural models have been recently widely used in the field of natural language process and have achieved very promising results~\cite{yin2016abcnn}. 
A neural attention mechanism equips a neural network with the ability to focus on a subset of its inputs when processing a large amount of information. Based on the network characteristics, attention neural networks have three main variants, i.e., global and local attention~\cite{luong2015effective}, hard and soft attention~\cite{shen2018reinforced}, and self-attention~\cite{zhang2019self}. 
Recently, Google proposed the Transformer model~\cite{vaswani2017attention} for natural language process tasks, which is the first transduction model relying entirely on self-attention to compute representations of its input and output. 

\subsection{Fuzz Testing}
\label{sec:bg2}
Software fuzzing in short generates mutants by modifying valid seed inputs to test a program~\cite{zalewski2014american}. The mutants are failed tests if they cause abnormal behaviors (e.g., crash the system under test) otherwise are passed tests.  
Coverage-guided fuzzing has been proposed and widely used to find many serious bugs in real software~\cite{aizatsky2016announcing}, in which a fuzzing process maintains an input data corpus for the program under consideration. 
Changes are made to those inputs according to some mutation procedure, and mutated inputs are kept in the corpus when they exercise new ``coverage''. 
Fuzzing testing techniques of traditional software leverage code coverage metrics that track which
lines of code have been executed and which branches have been taken~\cite{serebryanylibfuzzer,zalewski2014american}. 
However, these traditional fuzzing frameworks could not be directly applied to deep neural network-based
software due to the fundamental difference in the programming paradigm and the development process~\cite{xie2019deephunter}, i.e., 
a neural network run on different inputs will often execute the same lines of code and take the same branches, yet can produce significantly different behavior due to the difference in input values. 

To test deep neural networks, recently many coverage-guided fuzz testing frameworks have been proposed~\cite{xie2019deephunter,odena2019tensorfuzz,tian2018deeptest}, which applies the neuron coverage metrics to guide the fuzzing test to deep learning applications in the domain of image processing and they perform image transformations such as blurring and shearing to generate fuzzing inputs from seed images.  

==> Testing Machine Learning based Code Generation Models/sec/related.tex <==
\section{Related Work}
\label{sec:related}
\subsection{Testing Deep Learning Models}
\label{sec:rw_testDL}
In recent years, there are many studies on testing deep learning models~\cite{ma2018deepgauge,xie2019deephunter,tian2018deeptest,odena2019tensorfuzz,guo2018dlfuzz,pei2017deepxplore,wang2019adversarial,nejadgholi2019study}. 
Pei et al.~\cite{pei2017deepxplore} proposed DeepXplore to systematically find inputs that can trigger inconsistencies between multiple deep neural networks. 
They introduced neuron coverage as a systematic metric for measuring how much of the internal logic of a model have been tested. 
Tian et al.~\cite{tian2018deeptest} proposed DeepTest for failure detection on DNN-based Autonomous driving system. They adopted the neuron coverage metric as the criteria to generate synthetic inputs to test deep learning models. We use neuron coverage as guidance to our Mutation operator selection algorithm in our work. Ma et al.~\cite{ma2018deepgauge} purposed DeepGauge with 5 testing criterion for deep learning models, which extend the coverage metrics from neuron-level to layer-level. Odena et al.~\cite{odena2019tensorfuzz} presented TensorFuzz which applied fuzz-based coverage testing for deep learning systems. 
Nejadgholi~\cite{nejadgholi2019study} studied the oracle approximation issues in testing deep learning libraries. 
%The difference between our work and the above studies is that
%we apply neuron coverage as guidance while DeepHunter uses erroneous behavior for guidence. The difference between TensorFuzz and our work is that the TensorFuzz uses white noise as mutants while our mutants are dead code. Injecting dead code to the testing sample wil not change the semantic of the sample. 
Guo et al. \cite{guo2018dlfuzz} proposed DLFuzz, a differential fuzzing testing framework to guide deep learning systems exposing incorrect behaviors. 
%they also used neuron coverage as the fuzzing guidencee but they are maximizing the erroneous behaviour.
Xie et al.~\cite{xie2019deephunter} proposed DeepHunter, a fuzzing testing-based tool for testing deep learning models, in which they examined different types of seed selection strategy and test criteria.

The main difference between our work and the above studies is that most of the existing tools focus on general deep learning models in classic deep learning application domains, e.g., image processing, speech recognition, and natural language processing (NLP). While {\tool} is the first fuzzing framework for neural code models. 

%Researchers also explored other area of deep learning model testing\cite{kim2019guiding}\cite{sun2018testing}\cite{pei2017deepxplore}\cite{wang2018formal}\cite{sun2019deepconcolic}\cite{zhang2018deeproad}\cite{pei2017towards}\cite{du2019quantitative}\cite{ma2018deepmutation}\cite{tian2019testing}.
%There are studies on the criterion for testing deep learning systems such as Kim et al.\cite{kim2019guiding} and Sun et al. \cite{sun2018testing}. 
%Researchers also worked on different approaches to deep learning model testing problems including white box testing (Pei et al. \cite{pei2017deepxplore}), rigorous bounds calculation (Wang et al. \cite{wang2018formal}) and concolic-based testing (Sun et al. \cite{sun2019deepconcolic}). There exist studies that are similar to Deeptest, which focus on autonomous driving DL systems~\cite{zhang2018deeproad,gambi2019asfault,gambi2019asfault}. 

%Other relate work includes security analysis of deep learning systems~\cite{pei2017towards,du2019quantitative}, testing data quality measurement~\cite{ma2018deepmutation}, and bias errors testing~\cite{tian2019testing}.
\subsection{Adversarial machine learning.} 

Adversarial machine learning primarily focuses on generating adversarial examples to improve the performance of deep learning models~\cite{papernot2016limitations,cisse2017houdini,wang2019adversarial,gopinath2019symbolic,tuncali2018simulation,alcorn2019strike,alon2018general}. 
Gradient ascent-based adversarial example generation such as FGSM (Goodfellow et al. \cite{goodfellow2014explaining}) and BIM (Kurakin et al. \cite{kurakin2016adversarial}), which leverages the gradient of the model for finding adversarial example similar to the original input, has been widely used to accelerate the adversarial example generation problem for deep learning applications in the domains of image processing, speech recognition, and natural language processing. 

Recently, Yefet et al.~\cite{yefet2019adversarial} proposed DAMP, i.e., a gradient-based adversarial example generation technique, to generate adversarial examples for deep learning models in the domain of source code process. DAMP adopted two semantic preserving transformation operators, i.e., renaming variables and dead code inserting.  
Zhang et al.~\cite{zhang2020generating} proposed MHM that generated adversarial examples by renaming variables based on a sampling algorithm. Their experimental results demonstrate that MHM could effectively generate adversarial examples to attack the subject code process models. 
{Vahdat et al.~\cite{vahdat2021search} proposed a search-based testing framework for adversarial robustness testing. The differences to {\tool} are, firstly, out of the 10 operators {\tool} uses, there are 8 different operators compare to Vahdat et al.'s work. For the two similar operators (Renaming and Argument adding), {\tool} rename the variables with an 8-characters-length random string, while Vahdat et al.'s work uses the synonym of variable. Secondly, they used an evaluation metric derived from DeepMutation++~\cite{hu2019deepmutation++} to guide the mutation, while {\tool}  uses neuron coverage (NC) to guide the mutation.}
%\song{what's code coverage, do you use code coverage? what's deepmutation? what's the difference between them? please make the difference clear, you paper can be easily rejected because this!!!}\moshi{updated}



%To generate semantic preserving mutants for programs, except the two used transformations in the above studies, i.e., renaming variables and dead code inserting, {\tool} introduces eight more mutation operators (details are in Table~\ref{tab:opts}). 

%Gradient ascent-based adversarial example generation leverages the gradient of the model for finding adversarial example similar to the original input. In natural language processing, the generated adversarial example is usually replacing one of the tokens to a very close token in the embedding of the deep learning model. 
%Comparing to gradient ascent-based approach, our work used dead code mutants for adversarial example generation. We also simulated the behaviour of Gradient ascent-based approach with operator 10, one of the mutation operators of {\tool}.
%\vspace{-0.05in}

==> Testing Machine Learning based Code Generation Models/sec/result.tex <==
\section{Result Analysis}
\label{sec:result}
%\todo{Moshi}
\subsection{RQ1: Robustness of Neural Code Models}
\label{sec:rq1}
\input{table/rq1}

{\textbf{Approach.}} To answer this question, we re-use the original test sets of each model as a start point of the experiment. 
 %In {\neuralCodeSum}, we selected 1000 random samples from the original java test dataset in the GitHub repository of the project. In {\codeseq}, there are two types of test dataset, pre-processed dataset and source code dataset. we selected 1000 random samples from the java-small java source code test dataset using the download link provided in the Github repository of the project. The author of the {\codevec} is the same author who created {\codeseq}. In the {\codevec} Github repository, the author says the dataset we used in {\codeseq} is an extension dataset of {\codevec}, so we re-use the same dataset from {\codeseq} in {\codevec}.
 Specifically, for each studied neural code model, we randomly selected 1,000 samples from its original test dataset.
 For each sample, we randomly select one of the ten mutation operators from Table~\ref{tab:opts} and apply the mutation operator to the sample to generate a test. 
 Note that, given a sample program, it is possible that some mutation operators are not applicable, e.g., \textit{Op4}-duplication cannot be applied if a program does not have any assignment statements. If this happens, we continue to randomly select another mutation operator until one mutated program is generated. {Based on our experiments, at least one of the ten mutation operators can be applied to any of the samples.} Hence, we have 1,000 mutated programs from the 1,000 samples for each neural model.
 Then we evaluate the three pre-trained neural models with the 1,000 sample (i.e., \textit{1k original}) and the generated 1,000 mutants (i.e., \textit{1k mutants}). 

%For each model, we compare the performance of the model with 1000 randomly selected data from the test dataset provided by the model and 1000 mutants generated by {\tool} with one random selected mutation operator. We re-use the same measurement metrics of each model to measure the performance. We use BLEU measurement for {\neuralCodeSum} and F1 measurement for {\codeseq} and {\codevec} 
{\textbf{Results.}} Table~\ref{tab:rq1} shows the impacts of the simple perturbations on the performance of the neural models. In particular, we show the performance (either BLEU or F1) of the studied neural code models under two test datasets, i.e., before and after perturbations. For all the three neural code models, we notice the performance on \textit{1k mutants} decreases comparing to \textit{1k original}. Specifically, for {\neuralcodesum}, the BLEU score reduces 69.5\% (from 40.82 to 12.46). The F1 scores of {\codeseq} and {\codevec} reduce 5.9\% (from 71.16\% to 66.96\%) and 4.44\% (from 47.68\% to 45.56\%) respectively. 
%\jie{all performance use \% values (0-100)?}

Although all the three neural code models are susceptible to semantic-equivalent transformations; however, the impact of simple perturbations on the performance differs across the three neural models.  
As we can see the performance of  {\neuralcodesum} has declined significantly compared to {\codeseq} and {\codevec}. The main reason is that {\neuralcodesum} uses one %a~\jinqiu{one?} 
token sequence to represent %a method's body~\jinqiu
{the entire body of a method} and most of our proposed mutation operators can introduce new tokens into the method body, which impacts the representation vector and may further impact the performance of the model. 
While {\codeseq} and {\codevec} use both AST paths and AST token information to represent the entire body of a method, which are more stable than the token-based representation of {\neuralCodeSum}. 
%and half of our mutation operators (i.e., \textit{Op1}--\textit{Op4} and \textit{Op10}) do not affect the AST paths~\jinqiu{op1-op4 do impact the paths, no?}, 
Thus these two models are less susceptible to the perturbation introduced by random mutation. 

\mybox{
%Although achieving good performance %\jie{a little strong? NeuralCodeSum is not competitive...},all the three examined neural models of code still face the robust issues against random perturbations introduced by mutation.\jinqiu
{The studied neural code models face the robustness issues as their performance is negatively impacted by simple perturbations to test data. However, the negative impacts vary due to the use of different representations of code by each neural code model.}}

\subsection{RQ2: Comparison Across Different Mutation Operators}
\label{sec:rq2}
\input{figure/rq2_4_5_6}
\input{table/rq2_tab}
\input{table/rq2_nc}
%\input{table/rq2_nc_2}
%Table~\ref{tab:rq2_comp}
%To answer this question, we re-use the randomly collected 1000 testing sample in RQ1~\ref{sec:rq1}. 
%For each operator in {\tool}, we apply Opt1 to Opt10 to the test dataset T to generate the mutants MT1 to MT10. Then, we re-use the same evaluation scripts provided in each project and also re-use the pre-trained model in each paper for performance evaluation. Figure 2, Figure 3, Figure 4 shows the performance comparison of different operators on {\neuralCodeSum}, {\codeseq}, and {\codevec} respectively. The goal of this experiment is to compare the performance change introduced by each operator. 
%\jinqiu{Can use the approach and result style as well}
{\textbf{Approach.}} To answer this question, we use the same \textit{1K original} test sets for the three neural code models collected in RQ1 (Section~\ref{sec:rq1}). 
For each mutation operator in Table~\ref{tab:opts},  
we apply it on the \textit{1K original} test dataset to generate new test data. 
In total, we generate 10 new test sets, i.e., each test set is generated by applying one particular mutation operator.
We then examine the performance of the three neural code models on each of the new test sets.% and the results are shown in Table~\ref{tab:rq2_comp}. 
%\jie{break to a new para?}

We further examine the differences in terms of neuron coverage between each new test set and the original test set.  
In particular, we compute the neuron coverage of each test data, then calculate the average neuron coverage of each test set. Also, we calculate the average number of newly activated neurons of each test set based on a pairwise comparison between an original test data and a mutated one, i.e., the activated neurons in a mutated data that are not activated by the original data. 

%As some of the operators have lower neuron coverage compared to the \textit{1k original}, 
Moreover, we examine the difference between the two sets of activated neurons: one by an original test set, and the other by the mutated new test set. In particular, we calculate the Jaccard distance of each mutant sample against the original sample for each test set. % to check the difference between activated neurons of an operator and the \textit{1k original}. 
Given two sets of neurons $N1$ and $N2$ respectively. We measure their Jaccard distance by $1-\frac{N1\cap N2}{N1\cup N2}$. 
The Jaccard distance can be a value between 0 and 1, with 1 indicating no overlap at all and 0 indicating a complete overlap between the two sets.

\textbf{Results.} \textit{\textbf{Comparison Across the Ten Mutation Operators}}.
Overall, from the results shown in Table~\ref{tab:rq2_comp}, we observe that the performance of each model decreases on each of the 10 new test sets, i.e., the performance decline of {\neuralcodesum} ranges from 9.16\% (\textit{Op10}) to 85.25\% (\textit{Op5}) and the performance decline of {\codeseq} and {\codevec} ranges from 0.14\% (\textit{Op10}) to 21.33\% (\textit{Op6}) and 0.23\% (\textit{Op2}) to 16.01\% (\textit{Op9}) respectively. 
In addition, we can also see that the most effective mutation operators for each model are different, e.g., \textit{Op5} is the most effective mutation operator for {\neuralcodesum}, while for {\codeseq} and {\codevec}, the most effective mutation operator is \textit{Op6} and \textit{Op9} respectively. 
We further conduct the Mann-Whitney U test ($p < 0.05$) to compare the performance of the three neural code models under test data with (i.e., \textit{Op1}--\textit{Op10}) and without perturbations (i.e., original test set). 
The results suggest that the performance decline caused by simple perturbations is statistically significant in all the ten test sets and for all the three studied neural code models.
%from of the three models on each of the ten new test data is significantly lower than that on the \textit{1k original} dataset. 
%Note that, given a sample method, not all the mutation operators are applicable for it, e.g., Opt4 (duplication) does not work on methods that do not have assignment statements. Thus,  
%We compare the performance of each dataset with the same measurement used in the original paper of each model. As discussed in \ref{table/mutationOpts}, we label these dataset with the operator used to generate the mutants dataset, form Opt1 to Opt10. Also, we include the result of 1K original for comparison. Figure~\ref{fig:rq2_1}, Figure~\ref{fig:rq2_2}, and Figure~\ref{fig:rq2_3} shows the performance result for {\neuralCodeSum}, {\codeseq}, and {\codevec} respectively.

 
%we collected the neuron coverage for every sample in each of the ten test datasets, which are shown in 

Table~\ref{tab:rq2_nc} shows the comparison results across different mutation operators with regards to the impact on neuron coverage. 
Overall, the impact of each operator on neuron coverage varies across the studied neural code models. For example \textit{Op2}--\textit{Op7} significantly improve the neuron coverage on {\neuralCodeSum}, while decreasing the neuron coverage on {\codeseq}. This may be caused by the unique architecture of different models and properties of the test data. 
%~\jinqiu{also about the test data? Not sure.}
%\song{seems yes, the test data are different}
Interestingly, despite the decreased neuron coverage, we notice that all the mutation operators can activate new neurons compared to the original test sets. {This supports our design choice of using newly activated neurons instead of neuron coverage when guiding the search in fuzzing (line 12, Algorithm~\ref{alg:algorithm0})}.

%Compared to the neuron coverage achieved by the \textit{1k original} dataset, most of the ten new test datasets can improve the neuron coverage.  


%\jinqiu{one sentence to explain what jaccard distance means: if closer to 1, then?, closer to 0, then?}

Figure~\ref{fig:rq_2_ncs}, Figure~\ref{fig:rq_2_cs}, and Figure~\ref{fig:rq_2_nv} show the distribution of the Jaccard distance between the neuron coverage caused by each of the ten test datasets and the \textit{1k original} test data for {\neuralCodeSum}, {\codeseq}, and {\codevec} respectively. 
From these figures, we can see that the Jaccard distances vary for different operators and these results also confirm that different mutation operators activate different neurons at different rates.
% \jie{Are there any intuitive illustrations about the meaning of Jac distance, what 0.35 means (35\% of the sample difference?)? From these three figures, i could not see much information}
%\song{Some of the operators have low NC, thus we further check whether they have new neurons, the JACCARD was used to measure the difference between two sets of activated neurons}

%For all the studied models, the generated test cases increase the neuron coverage significantly—Wilcoxon nonparametric test confirms the statistical significance. 
%\jie{I could not understand here. from Table V, for example, with Op5 of code2seq, the coverage degrade. how can the test statistical? statistically lower ? Or This results is based on all the mutation operators (if this is the case, the logic is not so fluent since previous illustrations are about the separate operator?)?}
%\song{These are based on previous data, the data have been updated,}
%These results also show that different mutation operators activate different neurons at different rates.
%1000 mutants and the corresponding original sample for each mutation operations in {\neuralCodeSum}. The least effective operator in {\neuralCodeSum}, operator 10 in Figure~\ref{fig:rq2_4_plot} has the lowest Jaccard distribution comparing to other operators. The second least effecitve operator, operator 4, also shows less overall Jaccard distance comparing to the other operators. Figure~\ref{fig:rq2_5_plot} and Figure~\ref{fig:rq2_6_plot} also show that the Jaccard distance between the mutants and the original examples of each operators is positive static significant correlated with the performance impact of each mutation operators.

%\input{figure/rq2_4_plot}
%\input{figure/rq2_5_plot}
%\input{figure/rq2_6_plot}

%\subsubsection{\textbf{Op2}--\textbf{Op9} v.s. \textbf{Op1} and \textbf{Op10}}\
\input{table/rq3}
\textit{\textbf{Op2--Op9 v.s. Op1 and Op10}}.
As we described in Section~\ref{sec:step1}, operators \textit{Op1} and \textit{Op10} are proposed and used in prior studies~\cite{yefet2019adversarial,zhang2020generating} to generate adversarial examples for neural code models.
Regarding the effectiveness on reducing the performance of a neural model for code, five (i.e., \textit{Op5}--\textit{Op8}) of the eight operators (i.e., \textit{Op2}--\textit{Op9}) can outperform \textit{Op1} and all can outperform \textit{Op10} on {\neuralCodeSum}. We can also observe similar results on {\codeseq} and {\codevec}, i.e., five and four of the new proposed eight mutation operators can outperform \textit{Op1} respectively and \textit{Op10} is worse than all the eight new operators. 
%For other operators that can not outperform \textbf{Op1} and \textbf{Op10}, we further checked the 
In this work, we use all the ten mutation operators for the mutation-based test case generation, as each operator represents a unique type of semantic preserving transformations, which may trigger a different part of the examined neural code models, their different neuron coverage also confirms this.

%\jie{can we separate this subsection to subsubsections or with highlighted begin terms of important para. There are too much content. e.g., performance; neuron coverage; operator comparison ? (in the third part(last para), it is better to mention both performance and neuron role?)}
\mybox{All the ten mutation operators are shown to be effective in introducing perturbations that can significantly impact the performance of the studied neural code models. Our detailed analysis reveals that a mutated test set often activates a different set of neurons compared with the original test set. 
Last, the eight new mutation operators (i.e., \textit{Op2}--\textit{Op9}) are comparable or outperform the two operators (\textit{Op1} and \textit{Op10}) used in prior studies.}

%Operator 1, 5 to 9 have significant impact to the performance of the model while operator 2 to 4 and 10 has less significant impact to the performance

\subsection{RQ3: Effectiveness of {\tool}}
\label{sec:rq3}


\noindent{\textbf{Approach.}} We reuse the \textit{1k original} test data collected in RQ1 (Section~\ref{sec:rq1}) to explore the performance of the NC-guided mutation generation in {\tool}. 
For each test program in \textit{1k original} dataset,  
we use {\tool} and the baseline approach \textit{Random@3} to generate new test data respectively. 
Note that, the number of new test data generated by {\tool} has an upper bound, i.e., three times of the seed programs (see details in Section~\ref{sec:overall}). %~\jinqiu{check this is discussed}). 
The actual generated test set may contain less than the upper bound as the test data that does not activate new neurons is discarded. Meanwhile, \textit{Random@3} generates three new mutants for each seed program and yields a total of 3,000 generated programs. %~\jinqiu{this sentence is cut-off} 
Thus the number of generated mutants of these two approaches might not be the same. 
Then we examine the performance of the three models on the two new test sets (i.e., {\tool} and \textit{Random@3}) respectively. 
Last, we calculate the average neuron coverage of each test set and the average Jaccard distance between each mutated test data and its original test data (i.e., one seed program in the \textit{1k original} test set). %Results are shown in Table~\ref{tab:rq3}. 

%We again re-use the dataset T of each project in RQ1 for the experiment. There are two datasets we need to prepare in this experiment. The first one is Random@3 and the second one is NC-guided. In the first dataset preparation, for each sample in T, we perform mutation 3 times consecutively with 3 randomly selected mutation operators. i.e. we firstly select one random mutation operator K1 and mutate the sample with K1 to get the mutant M1. Then, we mutate M1 with one randomly selected mutation operator k2 to get the mutant M2, note that k1 and k2 can be the same operator. Then, we mutate M2 with one randomly selected mutation operator k3 to get the mutant M3. Again, k1, k2, and k3 can be the same operator. we collect the mutants M1, M2 and M3 generated from the above process, note Random@3. In the second dataset preparation, for each sample in T, we perform NC-guided operator selection algorithm and collect the mutants generated during the process. The key difference between random@3 AND NC-guided algorithm is, Random@3 randomly select one operator at each mutation of the sample while NC-guided algorithm select the operator that produce the best jaccard result. TABLE III shows the performance comparison of the two operator selection algorithms for three projects.

%To determine the effectiveness of operator selection algorithm in {\tool}, we compare the performance of the model with Random@3 mutants dataset and NC-guided mutants dataset. Table~\ref{tab:rq3} shows the performance comparison between Random@3 and NC-guided mutants dataset. 
\noindent{\textbf{Results.}}
As we can see from the results in Table~\ref{tab:rq3}, both {\tool} and \textit{Random@3} can  generate new tests that detect more {classification} errors on the neural code models. With the newly generated tests, the performance of each examined model decreases significantly and the decline rate can be up to 84.81\% (i.e., NC-guided on {\neuralCodeSum}). 
In terms of neuron coverage, NC-guided strategy ({\tool}) achieves a lightly higher neuron coverage than Random@3 and \textit{1k original}. Compared with the 10 test sets by applying each mutation operator individually (Table~\ref{tab:rq2_nc}), the NC-guided strategy also achieves the highest neuron coverage. Based on Jaccard distance, on average, the NC-guide strategy generates a new test set that activates more neurons compared to \textit{Random@3}. %collectively~\jinqiu{collectively? does that mean } achieve 48.95\%, 95.71\%, 75.23\% of neuron coverage for models {\neuralCodeSum}, {\codeseq}, and {\codevec} respectively. %thus increasing the coverage up to a\% b\%, and c\% w.r.t. the unguided baseline, i.e., \textbf{Random@3}. 
%Compared to {\tool} also achieves higher neuron coverage w.r.t. neuron coverage achieved by a single mutation operators (as shown in Table~\ref{tab:rq2_nc}). 
%\jie{It seems that the neuron coverage does not exert big difference for code2seq and neuralcodeSum, do we need to mention this aspect?}
%\song{updated}
%Test cases generated by NC-guided approach in {\tool} are more effective regarding introducing perturbations to decline the performance of the three models.

%This result shows that comparing to randomly select three operators and apply it to one sample consecutively three times, the NC-guided operator selection algorithm introduces additional performance drop. 

\mybox{By utilizing coverage-guided fuzzing strategy, {\tool} is more  effective in testing neural code models than the baseline \textit{Random@3}, i.e., a lower BLEU or F1 value, a higher neuron coverage, and a higher ratio of newly activated neurons.}


\subsection{RQ4: Usefulness of {\tool} on Improving Models}%\jie{retaining? should be retraining? maybe improving is better?}} 

\label{sec:rq4}


\noindent{\textbf{Approach.}} Similar to Deeptest~\cite{tian2018deeptest}, as a proof-of-concept, we showcase the usefulness of the mutated test data by using a subset of the entire training data. In particular, we first train the three neural models with 10k randomly selected original training data from scratch. We reuse the validation dataset provided by each of the three models during the training process. 
%A complete retraining with the complete original training data as the training process could take weeks. 
Then for each neural code model, we apply {\tool} and \textit{Random@3} on the selected 10K training data to generate two new test sets. Combining the mutated test sets and the 10K randomly selected training data, we obtain two sets of enhanced training datasets, i.e., one enhanced by {\tool} and one by \textit{Random@3}. 
We then re-train each of the three models with the two enhanced training datasets respectively. 
Finally, we evaluate these re-trained models on the \textit{1K original} test dataset. %and the enhanced \textit{1k original}, i.e., \add{1k original and 1k mutants generated from it via randomly selected mutation operators}.
%the mutated test set by {\tool} (RQ3). %Results are shown in Table~\ref{tab:rq4}.
\input{table/rq4}
\noindent{\textbf{Results.}} Table~\ref{tab:rq4} compares the performance across three types of training sets, i.e., original data, original data enhanced by Random@3 strategy, and original data enhanced by {\tool}. %\jinqiu{Need an update after Table VII is complete.} 
As we can see from the table, in all cases, the
performance of the re-trained model improved significantly over the original model and the improvements are 35.15\% on {\neuralCodeSum}, 8.83\% on {\codeseq}, and 34.14\% on {\codevec}.  

%\jie{the improvement of code2seq and code2vec is not so obvious? especially compared with the random method, 23.16 - 23.66, 15.13 - 15.48? Do we need to explain the reasons? or list the performance improvement of using variable rename (which is similar with this case?) to state this improvement is comparable in other scenarios (e.g., use the results from image classification improvement)? 
%Otherwise, i think this point can be argued by the reviewers.}
%\song{updated to the latest experiments}

%\jie{another point, i am not quite sure. if we use another 1K test dataset to evaluate the re-trained model, can the performance improvement be larger? Just curious.}
%To determine whether {\tool} improves the neural program summerization model. we re-train the model with 10000 random samples from the training dataset and compare the performance with the model re-trained with the 10000 random samples plus the mutants generated with two different algorithms from these 10000 random samples. For each model, we randomly select 10000 training examples form the java training dataset, note TrData. Then we apply Random@3 algorithm to TrData and collect the generated mutants as Random@3. Then we apply NC-guided algorithm to TrData and collect mutants as Adversarial. We re-train the model from scratch with TrData, TrData + Adversarial, and TrData + Random. Then we re-use the evaluation scripts provided in each projects for performance evaluation. TABLE IV shows the performance result comparison of the experiments.
%Table~\ref{tab:rq4}
\mybox{Performance of the three neural code models can be improved 35.15\% on {\neuralCodeSum}, 8.83\% on {\codeseq}, and 34.14\% on {\codevec} by retraining the models with synthetic data generated by {\tool}.} 

==> Testing Machine Learning based Code Generation Models/sec/setup.tex <==
\section{Experiment Setup}
\label{sec:experiment}
We run all the experiments on the Google Cloud Computing Platform. Specifically, we use two n1-highmem-2 virtual central processing unit (vCPU) with 13 gigabyte memory in total and one NVIDIA Tesla T4 GPU as hardware of our experiment machine. 
We use PyTorch 1.4 for running {\neuralCodeSum}, TensorFlow 1.15 for {\codeseq}, and TensorFlow 2.1 for {\codevec}. 
%\Moshi{configuration added. pls review}

\subsection{Subject Models and Datasets} 
\label{sec:sub}

\subsubsection{Studied Models}
\label{sec:smodels}

In this work, to evaluate {\tool}, we use three state-of-the-art neural code models that adopt different neural network characteristics, i.e., {\neuralCodeSum}~\cite{ahmad2020transformer},  {\codeseq}~\cite{alon2018code2seq}, and {\codevec}~\cite{alon2019code2vec}. 
For our experiments, we reuse the pre-trained models of the three studied neural code models, which are released in their papers.
{All the three models are common in learning code embedding from large-scale data and generating a high-level summary given a method. However, the three models are different in many aspects. First, they utilize different model architectures. Second, they have different representations of code. Third, the level of details in the generated summaries from the three models is different, i.e., {\neuralCodeSum} generates full English sentence as output while {\codeseq} and {\codevec} produce  the name of the method.} %@moshi, are the above correct? Anything else? You can add ", i.e., ..." to expand each point a bit.} 
We briefly describe the details of the three models below.
%\todo{Moshi: The aboves are correct.}

%First, they utilize different model architectures, i.e. {\neuralCodeSum} uses Tansformer architecture, {\codeseq} uses encoder-decoder architecture, and {\codevec} uses AST path based bag-of-word embedding. Second, they have different representations of code, i.e. {\neuralCodeSum} represent each token as a word from the dictionary while {\codeseq} and {\codevec} represent each token as an AST path to the token. Third, the level of details in the generated summaries from the three models is different, i.e. {\neuralCodeSum} generates full English sentence as output while {\codeseq} and {\codevec} produce  the name of the method.


\noindent \textbf{\neuralCodeSum}~\cite{ahmad2020transformer} uses  Transformer~\cite{ahmad2020transformer} (consists of stacked multi-head attention and parameterized linear transformation layers for both the encoder and decoder) to generate a natural language summary
given a piece of source code. Both the code and
the summary is a sequence of tokens that are represented by a sequence of vectors. To allow the Transformer to utilize the order information of source code tokens, {\neuralCodeSum} encodes both the absolute position and pairwise relationship of source code tokens.

\noindent \textbf{\codeseq}~\cite{alon2018code2seq} uses an encoder-decoder architecture to encode paths node-by-node and generate label as sequences. In {\codeseq}, the encoder represents a method’s body as a set of AST paths where each path is compressed to a fixed-length vector using a bi-directional LSTM which encodes paths node-by-node. 
The decoder uses attention to select relevant paths while decoding and predicts sub-tokens of target sequence at each step when generating the method’s name. 

\noindent \textbf{\codevec}~\cite{alon2019code2vec} %uses a bag of AST paths to represent the source code. 
proposes a path-based attention model for learning vectors for arbitrary-sized snippet of code. The model allows to embed a program into a continuous space.
Specifically it first extracts syntactic paths from within a code snippet, i.e., ASTs, and then it represents them as a bag of distributed vector representations.%, and finally it uses 
An attention network will be used to compute a learned weighted average of the path vectors in order to produce a single code vector. 
%Each path consists of a pair of terminals in the abstract syntax tree and their corresponding path between them in the AST. 
%The path, along with source and destination terminals are mapped into its vector embeddings which are learned jointly with other network parameters during training. 
%The above vectors of each path-context are then concatenated to a single context vector using a fully connected layer which is learned during training with the network. 
%An attention vector is also learned with the network which is used to score each path-context and aggregate multiple path-contexts to a single code vector representing the method’s body. 
%After that, the model predicts the probability of each target method’s name given the code vector of the method’s body.

\subsubsection{Dataset}
\label{sec:sdata}
\input{table/dataset}

We perform our experiments using the original datasets associated with each of the three studied neural code models. 
Table~\ref{tab:data} lists the basic statistics of the three datasets. Specifically, the dataset of {\neuralCodeSum} contains 9.7K open source Java projects hosted in GitHub and each of the projects has at least 20 stars. 87.1k methods that have JavaDoc comments were collected. 
%\todo{Moshi: update these numbers}
{\codeseq} created three Java datasets, which are different in size, the popularity of the open-source software where the data is from, and the distribution of training, validation and testing. Among the three Java datasets by {\codeseq}, we decided to use one, i.e., \textit{Java-small}. Despite its relatively small size among the three, it is commonly used by prior studies~\cite{allamanis2016convolutional, alon2019code2vec}, including {\codevec}. Also, all the projects in \textit{Java-small} are large-scale and mature open-source software, in comparison with the other two datasets (i.e., many are from smaller and less popular projects). 
%{\codevec} and {\codeseq} use the same datasets provided by {\codeseq}. 
\textit{Java-small} contains 11 relatively large Java projects 9 for training, 1 for validation, and 1 for testing. Overall, it contains about 772.9K methods. 
%The compressed size is about 366MB and the extracted size is about 1.9GB.

\subsection{Evaluation Metrics}
\label{sec:metrics}
We use the same evaluation metrics with the original papers of {\neuralCodeSum}, {\codeseq}, and {\codevec} for comparison purpose.
{\neuralCodeSum} 
adopts BLEU~\cite{papineni2002bleu} to evaluate its performance on predicting the summarization of programs. BLEU is widely used to assess the quality of machine translation systems~\cite{cho2014learning}.  %It is defined as the geometric mean of n-gram (for BLEU, n=1,2,3,4) matching precision scores multiplied by a length brevity penalty factor.  
BLEU's output is always a number between 0 and 1. This value indicates how similar the predicting summarization is to the ground-truth, with values closer to 1 representing more similar. 

Differently, {\codevec} and {\codeseq} used precision, recall, and F1 for measuring performance.
%\moshi{better make these equations larger, instead of inline}
Precision and Recall are computed in a per-subtoken basis. F1 is the weighted average of Precision and Recall. %This is based on the assumption that the quality of a method name prediction mainly depend on the sub-words that were used to compose it. 
%Precision and Recall are composed of three numbers, i.e., true positive, false positive, and false negative. 
%We show the formulas below.%~\jinqiu{The formulas can be placed inline.}
%Precision is calculated by ${true\ positive}/({true\ positive + false\ positive})$, Recall is ${true\ positive}/({true\ positive + false\ negative})$, and F1 is ${2*Precision*Recall}/({Precision + Recall})$.
%begin{equation}
%F1 = \frac{2*Precision*Recall}{Precision + Recall}
%\end{equation}

%To calculate precision and recall, each method name (i.e., a predicted one and the ground-truth one), are first split into a vector of words following camel case. 
%The true positive is the number of predicted words that are also in the word vector of ground-truth name, while false positive is the number of predicted words that are not in the word vector of the ground-truth name.  
%The false negative is the number of words in the ground-truth name that are not in the predicted name. 

\subsection{Baseline}
\label{sec:baselines}
\subsubsection{Baseline for Mutation Operators} 

As two of the ten mutation operators are used in prior studies~\cite{yefet2019adversarial,zhang2020generating}, namely \textit{Op1} (i.e., dead code inserting) and \textit{Op10} (i.e.,renaming). 
We treat them as baselines to evaluate the eight new mutation operators, i.e., \textit{Op2}-- \textit{Op9}.  

\subsubsection{Baseline for NC-Guided Test Generation} 
{\tool} uses neuron coverage to guide the test generation via the combination of mutation operators. 
To evaluate the effectiveness of {\tool} we have also designed a baseline approach that generates tests without neuron coverage guidance, i.e., \textit{Random@K}, which randomly picks $K$ mutation operators to generate mutants as tests.  
$K$ indicates the maximum number of mutations tries on a seed program. As we described in Section~\ref{sec:approach}, {\tool} limits the maximum number of mutation tries to three, thus in our experiment we also set $K$ to three. 
Given a seed program, \textit{Random@3} 
first randomly selects a mutation operator $op_{i}$ and mutate the sample to get the mutant $M1$. 
Then, it mutates $M1$ with another randomly selected mutation operator $op_{j}$ to get a new mutant $M2$, after that it further mutates $M2$ with a randomly selected mutation operator $op_{h}$ to generate a new mutant M3. Through the process, $op_{i}$, $op_{j}$, and $op_{h}$ can be the same operator.
\textit{Random@3} produces a total of 3 mutants for a given seed program.  
% \jie{The reviewers might argue we did not compare with the baselines proposed in previous approach. Can we add an explanation somewhere to say that Op1, Op10 are actually the baselines ? }

\subsection{Research Questions}
\label{sec:rqs} 
We have implemented {\tool} as a self-contained fuzz testing framework in Python based on deep learning framework Keras, TensorFlow, and Pytorch. With {\tool}, we perform a large-scale comparative study to answer the following four research questions. 


\vspace{4pt}
\noindent  \textbf{RQ1:} \textit{Are the neural code models robust against simple perturbations?}

Robustness has been extensively studied in classic deep learning application domains, e.g., image processing, speech recognition, and NLP. Many of these deep learning models have been shown that they could be easily attacked by simple perturbations. As the first study on exploring the robustness of neural code models, in this RQ, we explore whether they also suffer similar issues.
%and re-use the same evaluation scripts provided in the projects. We also re-use the same performance metric in each of the original papers. 
 %In {\neuralCodeSum}, we re-use the pre-trained model in the paper provided by the author of {\neuralCodeSum}. The {\neuralCodeSum} paper uses BLEU to evaluate the performance of the model. We re-use the evaluation script provided by the {\neuralCodeSum} project with the dataset T to get the BLEU score of T, note 1K original.
 %Then, We run the same evaluation script with MT to get the BLEU score of MT, note 1K mutants. 
 %In {\codeseq}, we use the model java-large-model-iter52, the same model used in the {\codeseq} paper, for performance evaluation. We re-use the evaluation scripts in code2seq to the get F1 score of dataset T, note 1K original. Then, we re-use the evaluation scripts in code2seq to the get F1 score of dataset MT, note 1K mutants .In {\codevec}, we use the model java14-model-saved-model-iter8, the same model used in the {\codevec} paper, for performance evaluation. We re-use the evaluation scripts in {\codevec} to the get F1 score of dataset T, note 1K original. Then, we re-use the evaluation scripts in {\codevec} to the get F1 score of dataset MT, note 1K mutants. TABLE II shows the performance comparison of the 6 result.
 
\vspace{4pt}
\noindent  \textbf{RQ2:} \textit{What is the effectiveness of each mutation operator?}

%We propose ten mutation operators (Table~\ref{tab:opts}) for mutating programs in a semantic-preserving manner. 
This RQ illustrates the effectiveness of each mutation operator (a total of ten in Table~\ref{tab:opts}) regarding its capability of introducing perturbations that can affect the performance of neural code models and activating different neurons. 
%Furthermore, two mutation operators are used in prior studies~\cite{yefet2019adversarial,zhang2020generating}, namely \textit{Op1} (i.e., dead code inserting) and \textit{Op10} (i.e., renaming). 
Furthermore, this RQ also examines the effectiveness of the two baseline operators (i.e., \textit{Op1} and \textit{Op10}) in comparison to other eight new mutation operators. 

\vspace{4pt}
\noindent  \textbf{RQ3:} \textit{What is the effectiveness of the NC-guided test generation in {\tool}?}

 {\tool} uses neuron coverage to guide the search for new tests that are continuously transformed through multiple mutation operators. This RQ explores the performance of {\tool} and compares it with our constructed baseline, i.e., \textit{Random@3}.

%We again re-use the dataset T of each project in RQ1 for the experiment. There are two datasets we need to prepare in this  experiment. The first one is Random@3 and the second one is NC-guided. In the first dataset preparation, for each sample in T, we perform mutation 3 times consecutively with 3 randomly selected mutation operators. i.e. we firstly select one random mutation operator K1 and mutate the sample with K1 to get the mutant M1. Then, we mutate M1 with one randomly selected mutation operator k2 to get the mutant M2, note that k1 and k2 can be the same operator. Then, we mutate M2 with one randomly selected mutation operator k3 to get the mutant M3. Again, k1, k2, and k3 can be the same operator. we collect the mutants M1, M2 and M3 generated from the above process, note Random@3. In the second dataset preparation, for each sample in T, we perform NC-guided operator selection algorithm and collect the mutants generated during the process. The key difference between random@3 AND NC-guided algorithm is, Random@3 randomly select one operator at each mutation of the sample while NC-guided algorithm select the operator that produce the best jaccard result. TABLE III shows the performance comparison of the two operator selection algorithms for three projects.

\vspace{4pt}
\noindent  \textbf{RQ4:} \textit{Is {\tool} useful for improving neural code models?}

This RQ explores whether the synthetic programs can improve the neural code models, i.e., whether retraining with  with \tool's synthetic programs can make these models more robust. 
%To determine whether {\tool} improves the neural program summerization model. we re-train the model with 10000 random samples from the training dataset and compare the performance with the model re-trained with the 10000 random samples plus the mutants generated with two different algorithms from these 10000 random samples. For each model, we randomly select 10000 training examples form the java training dataset, note TrData. Then we apply Random@3 algorithm to TrData and collect the generated mutants as Random@3. Then we apply NC-guided algorithm to TrData and collect mutants as Adversarial. We re-train the model from scratch with TrData, TrData + Adversarial, and TrData + Random. Then we re-use the evaluation scripts provided in each projects for performance evaluation. TABLE IV shows the performance result comparison of the experiments.



==> Testing Machine Learning based Code Generation Models/table/dataset.tex <==
\begin{table}[t!]
\centering
%\setlength{\tabcolsep}{2pt}
\caption{ Experimental datasets. `Pro' is the number of projects.}%\jinqiu{Are these training sets?}}
\label{tab:data}
\scalebox{0.8}{
\begin{tabular}{lcccccc}
\toprule \hline
\multicolumn{1}{c}{Model}       & Language   & \multicolumn{1}{l}{\#Pro} &  \multicolumn{1}{l}{\#Training}& \multicolumn{1}{l}{\#Validation}& \multicolumn{1}{l}{\#Test}& \multicolumn{1}{l}{\#Method} \\ \hline
{\neuralCodeSum} & Java            & 9.7k     &  69.7k      &    8.7k    &         8.7k           & 87.1K                         \\ \hline
{\codeseq}       & \multirow{2}{*}{Java}  & \multirow{2}{*}{11}     & \multirow{2}{*}{692.0k} &\multirow{2}{*}{23.8k}   &\multirow{2}{*}{57.1k}        & \multirow{2}{*}{772.9K}         \\ 
{\codevec}       &                       &                                &                               \\ \bottomrule \hline
\end{tabular}
}
\end{table}

==> Testing Machine Learning based Code Generation Models/table/ds_1.tex <==
\begin{table}[t!]
\centering
\caption{\small Statistics of the impact of the position independent mutation operations used in this study.
\textbf{Performance Distribution} indicates the distribution of the performance of a model with 10 different test datasets generated by a mutation operator. 
\textbf{SD} is the standard deviation of the performance of a model with different test datasets. }
\label{tab:ds_1}
\begin{tabular}{lccc}
\hline
\textbf{Model}   & \textbf{Operator}   & \textbf{Performance Distribution} & \textbf{SD} \\
& & Average ($\pm$ Range) & \\\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}{\neuralCodeSum}\\ BLEU(\%)\end{tabular}}       & Op1& 7.10 ($\pm0.28$)     &  0.16   \\ 
 & Op5& 5.78 ($\pm0.43$)     &  0.27    \\ 
 & Op6& 5.88 ($\pm0.38$)     &  0.23   \\ 
 & Op7& 5.92 ($\pm0.40$)     &  0.24    \\ 
 & Op8& 6.50 ($\pm0.00$)     &  0.00     \\   
 & Op9& 6.61 ($\pm0.00$)     &  0.00        \\ \hline \hline
%  & Opt10&  34.97($\pm0.00$)    &  0.00   \\ \hline \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}{\codeseq}\\ F1(\%)\end{tabular}}            & Op1& 65.05 ($\pm1.47$)    &    0.01  \\ 
 & Op5& 63.98 ($\pm1.02$)    &    0.006  \\ 
 & Op6& 62.09 ($\pm1.56$)    &    0.009  \\  
 & Op7& 64.02 ($\pm1.26$)    &    0.008  \\ 
 & Op8& 64.65 ($\pm1.34$)    &    0.008  \\ 
 & Op9& 65.66 ($\pm1.14$)    &    0.008  \\   \hline \hline
% & Opt10&  0.66 ($\pm0.00$)    &   0.003   \\ \hline \hlinevec
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}{\codevec}\\ F1(\%)\end{tabular}}            & Op1& 60.51 ($\pm2.46$)    &    0.02  \\
 & Op5& 59.95 ($\pm2.01$)    &   0.01  \\ 
 & Op6& 57.81 ($\pm2.44$)   &    0.01  \\
 & Op7& 60.34 ($\pm1.29$)   &    0.009  \\ 
 & Op8& 58.42 ($\pm2.14$)   &    0.01  \\  
 & Op9& 54.62 ($\pm1.91$)  &    0.01  \\ \hline
% & Opt10 & 0.61($\pm0.006$)  &  0.003  \\ \hline
\end{tabular}
\vspace{-0.1in}
\end{table}


==> Testing Machine Learning based Code Generation Models/table/ds_2.tex <==
\begin{table}[t!]
\centering
\caption{ \small The distribution of selected mutation operators on the three models.}
\label{tab:ds_2}
\begin{tabular}{cccc}
\hline
\textbf{Operator} & \textbf{{\neuralCodeSum}} & \textbf{{\codeseq}} & \textbf{{\codevec}} \\ \hline
Op1     &    9.05\%                &    6.46\%           &     0.87\%     \\ 
Op2     &    8.39\%                &    10.83\%          &     15.30\%     \\ 
Op3     &    4.43\%                &    2.13\%           &     2.63\%     \\ 
Op4     &    2.82\%                &    0.63\%           &     1.23\%     \\ 
Op5     &    \textbf{15.79\%}      &    \textbf{19.00\%} &     \textbf{26.07\%}   \\ 
Op6     &    14.83\%               &    14.83\%          &     11.03\%    \\ 
Op7     &    13.97\%               &    9.13\%           &     5.53\%    \\ 
Op8     &    12.73\%               &    18.33\%          &     16.67\%   \\ 
Op9     &    13.21\%               &    16.50\%          &     19.37\%   \\ 
Op10    &    4.74\%                &    1.10\%          &     1.30\%     \\ \hline
\end{tabular}
\vspace{-0.1in}
\end{table}


==> Testing Machine Learning based Code Generation Models/table/mutationOpts.tex <==
\begin{table}[t!]
\centering
\caption{Ten Semantic-Preserving Mutation Operators Applied in {\tool}.}
\label{tab:opts}
\setlength{\tabcolsep}{3pt}
\scalebox{0.8}{
\begin{tabular}{lll}
\toprule \hline
\textbf{NO.} & \textbf{Operator name}  & \textbf{Description}  \\ \hline
Op1~\cite{yefet2019adversarial} & dead store            & Inserting unused variable declarations\\ \hline

Op2 & numerical obfuscating & \begin{tabular}[c]{@{}l@{}}Obfuscating the numerical variables via\\ adding/deleting a same numerical value\end{tabular} \\ \hline
Op3 &adding zero & \begin{tabular}[c]{@{}l@{}}Obfuscating the numerical values via\\ adding zero \end{tabular} \\ \hline

Op4 & duplication          & Duplicating assignment statements\\ \hline
Op5 & unreachable \textit{if}   & Inserting unreachable \textit{if} statements \\ 
Op6 & unreachable \textit{if-else}  & Inserting unreachable \textit{if-else} statements \\ 
Op7 & unreachable \textit{switch}  & Inserting unreachable  \textit{switch} statements \\ 
Op8 & unreachable \textit{for}      & Inserting unreachable  \textit{for} statements \\ 
Op9 & unreachable \textit{while}   & Inserting unreachable  \textit{while} statements \\ \hline
Op10~\cite{yefet2019adversarial,zhang2020generating} & renaming              & Renaming user-defined variables \\ \bottomrule \hline
\end{tabular}
}
\end{table}

==> Testing Machine Learning based Code Generation Models/table/rq1.tex <==
\begin{table}[t!]
\centering
\caption{ The results of testing the three neural code models on the test data before (i.e., \textit{1K original}) and after (\textit{1K mutants}) introducing simple perturbations.}
\label{tab:rq1}

\begin{tabular}{ccr}
\toprule \hline
\textbf{Model}         & \textbf{Test data} & \textbf{Performance (\%)} \\ \hline
\multirow{2}{*}{\neuralCodeSum} & \textit{1K original}   &  BLEU = 40.82 \\ %\cline{2-3}  
           & \textit{1K mutants}    &  BLEU = 12.46    \\ \hline
\multirow{2}{*}{\codeseq}   & \textit{1K original}   &  F1 = 71.16  \\ %\cline{2-3} 
           & \textit{1K mutants}    &  F1 = 66.96    \\ \hline
\multirow{2}{*}{\codevec}   & \textit{1K original}   &  F1 = 47.68    \\ %\cline{2-3} 
           & \textit{1K mutants}    &  F1 = 45.56    \\ 
           \bottomrule \hline
\end{tabular}
\vspace{-0.1in}
\end{table}

==> Testing Machine Learning based Code Generation Models/table/rq2_nc.tex <==
\begin{table}[t!]
\centering
\caption{ The average neuron coverage of the test sets generated using different mutation operators. Numbers in the brackets are the average number of newly activated neurons.}
%\todo{Moshi:fill the number of new activated neurons }}%\jie{I seems that this figure is similar with Table IV. do we use the same format? XX (YY\% up or down?)}}
%\todo{moshi}}
\label{tab:rq2_nc}
\begin{tabular}{cccc}
\toprule \hline
   & \textbf{{\neuralCodeSum}} & \textbf{{\codeseq}} & \textbf{{\codevec}} \\ \hline
\multicolumn{1}{l}{ Original} &44.94\%&   90.79\% &  60.99\%\\ \hline
\multicolumn{1}{l}{Op1}&\textbf{47.33\%} (722.80)   &\textbf{91.46\%} (39.08)&  \textbf{61.48\%} (19.13)\\ %\hline
\multicolumn{1}{l}{Op2}&\textbf{47.07\%} (702.65)         &   90.73\% (16.72) &  \textbf{61.00\%} (32.90)\\ %\hline
\multicolumn{1}{l}{Op3}&\textbf{47.06\%} (702.32)         &   90.76\% (11.17) &  60.98\% (25.12)\\ %\hline
\multicolumn{1}{l}{Op4}&\textbf{45.75\%} (700.31)         &   90.68\% (19.80)&  \textbf{61.17\%} (31.00)\\ %\hline
\multicolumn{1}{l}{Op5}&\textbf{47.55\%} (745.05)         &   88.61\% (55.83)&  \textbf{62.37\%} (50.82)\\ %\hline
\multicolumn{1}{l}{Op6}&\textbf{47.49\%} (742.95)         &   89.53\% (55.44) &  \textbf{62.33\%} (44.40)\\ %\hline
\multicolumn{1}{l}{Op7}&\textbf{47.48\%} (741.40)         &   88.98\% (53.99) &  \textbf{62.04\%} (41.91)\\ %\hline
\multicolumn{1}{l}{Op8}&\textbf{48.11\%} (768.31)&   \textbf{91.36\%} (52.39) &  \textbf{62.66\%} (48.44)\\ %\hline
\multicolumn{1}{l}{Op9}&\textbf{48.10\%} (772.08)   &   \textbf{91.50\%} (53.21) &  \textbf{62.70\%} (49.41)\\ %\hline
\multicolumn{1}{l}{Op10}&44.91\% (459.86)   &   \textbf{90.86\%} (21.82) &  60.97\% (25.17)\\ \bottomrule \hline
\end{tabular}
\vspace{-0.1in}
\end{table}
























\begin{comment}
\begin{table}[t!]
\centering
\caption{Neuron coverage of different mutation operators. Values are in percentage. Numbers in the brackets are the difference.}%\jie{I seems that this figure is similar with Table IV. do we use the same format? XX (YY\% up or down?)}}
%\todo{moshi}}
\label{tab:rq2_nc}
\begin{tabular}{c|c|c|c|}
\cline{2-4}
   & \textbf{{\neuralCodeSum}} & \textbf{{\codeseq}} & \textbf{{\codevec}} \\ \hline
\multicolumn{1}{|l|}{Original} &44.94&   90.79 &  60.99\\ \hline
\multicolumn{1}{|l|}{Op1}&\textbf{47.33 (5.32\%$\uparrow$)} &\textbf{1.46 (0.74\%$\uparrow$)}&  \textbf{61.48 (0.80\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op2}&\textbf{47.07 (4.74\%$\uparrow$)}&   90.73 (0.06\%$\downarrow$) &  \textbf{61.00 (0.02\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op3}&\textbf{47.06 (4.72\%$\uparrow$)}&   90.76 (0.03\%$\downarrow$) &  60.98 (0.02\%$\downarrow$)\\ \hline
\multicolumn{1}{|l|}{Op4}&\textbf{45.75 (1.80\%$\uparrow$)}   &   90.68 (0.12\%$\downarrow$)&  \textbf{61.17 (0.29\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op5}&\textbf{47.55 (5.81\%$\uparrow$)}   &   88.61 (2.40\%$\downarrow$)&  \textbf{62.37 (2.26\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op6}&\textbf{47.49 (5.67\%$\uparrow$)}   &   89.53 (1.38\%$\downarrow$) &  \textbf{62.33 (2.19\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op7}&\textbf{47.48 (5.65\%$\uparrow$)}   &   88.98 (1.99\%$\downarrow$) &  \textbf{62.04 (1.72\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op8}&\textbf{48.11 (7.05\%$\uparrow$)}  &   \textbf{91.36 (0.63\%$\uparrow$)} &  \textbf{62.66 (2.74\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op9}&\textbf{48.10 (7.03\%$\uparrow$)}   &   \textbf{91.50 (0.78\%$\uparrow$)} &  \textbf{62.70 (2.80\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op10}&44.91 (0.07\%$\downarrow$)   &   \textbf{90.86 (0.07\%$\uparrow$)} &  60.97 (0.03\%$\downarrow$)\\ \hline
\end{tabular}
\end{table}
\end{comment}

==> Testing Machine Learning based Code Generation Models/table/rq2_nc_2.tex <==
\begin{table}[t!]
\centering
\caption{Neuron coverage of different mutation operators. Values are in percentage. Numbers in the brackets are the number of new activated neurons.
\todo{Moshi:fill the number of new activated neurons }}%\jie{I seems that this figure is similar with Table IV. do we use the same format? XX (YY\% up or down?)}}
%\todo{moshi}}
\label{tab:rq2_nc_2}
\begin{tabular}{c|c|c|c|}
\cline{2-4}
   & \textbf{{\neuralCodeSum}} & \textbf{{\codeseq}} & \textbf{{\codevec}} \\ \hline
\multicolumn{1}{|l|}{Op1}&\textbf{722.80 }   &   \textbf{39.08}  &  \textbf{19.13 }\\ \hline
\multicolumn{1}{|l|}{Op2}&\textbf{702.65 }   &           16.72   &  \textbf{32.90 }\\ \hline
\multicolumn{1}{|l|}{Op3}&\textbf{702.32 }   &           11.17   &          25.12  \\ \hline
\multicolumn{1}{|l|}{Op4}&\textbf{700.31 }   &           19.80   &  \textbf{31    }\\ \hline
\multicolumn{1}{|l|}{Op5}&\textbf{745.05 }   &           55.83   &  \textbf{50.82 }\\ \hline
\multicolumn{1}{|l|}{Op6}&\textbf{742.95 }   &           55.44   &  \textbf{44.40 }\\ \hline
\multicolumn{1}{|l|}{Op7}&\textbf{741.40 }   &           53.99   &  \textbf{41.91 }\\ \hline
\multicolumn{1}{|l|}{Op8}&\textbf{768.31 }   &   \textbf{52.39 } &  \textbf{48.44 }\\ \hline
\multicolumn{1}{|l|}{Op9}&\textbf{772.08 }   &   \textbf{53.21 } &  \textbf{49.41 }\\ \hline
\multicolumn{1}{|l|}{Op10}&       459.86     &   \textbf{21.82 } &          25.17 \\ \hline
\end{tabular}
\end{table}








\begin{comment}
\begin{table}[t!]
\centering
\caption{Neuron coverage of different mutation operators. Values are in percentage. Numbers in the brackets are the difference.}%\jie{I seems that this figure is similar with Table IV. do we use the same format? XX (YY\% up or down?)}}
%\todo{moshi}}
\label{tab:rq2_nc}
\begin{tabular}{c|c|c|c|}
\cline{2-4}
   & \textbf{{\neuralCodeSum}} & \textbf{{\codeseq}} & \textbf{{\codevec}} \\ \hline
\multicolumn{1}{|l|}{Original} &44.94&   90.79 &  60.99\\ \hline
\multicolumn{1}{|l|}{Op1}&\textbf{47.33 (5.32\%$\uparrow$)} &\textbf{1.46 (0.74\%$\uparrow$)}&  \textbf{61.48 (0.80\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op2}&\textbf{47.07 (4.74\%$\uparrow$)}&   90.73 (0.06\%$\downarrow$) &  \textbf{61.00 (0.02\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op3}&\textbf{47.06 (4.72\%$\uparrow$)}&   90.76 (0.03\%$\downarrow$) &  60.98 (0.02\%$\downarrow$)\\ \hline
\multicolumn{1}{|l|}{Op4}&\textbf{45.75 (1.80\%$\uparrow$)}   &   90.68 (0.12\%$\downarrow$)&  \textbf{61.17 (0.29\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op5}&\textbf{47.55 (5.81\%$\uparrow$)}   &   88.61 (2.40\%$\downarrow$)&  \textbf{62.37 (2.26\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op6}&\textbf{47.49 (5.67\%$\uparrow$)}   &   89.53 (1.38\%$\downarrow$) &  \textbf{62.33 (2.19\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op7}&\textbf{47.48 (5.65\%$\uparrow$)}   &   88.98 (1.99\%$\downarrow$) &  \textbf{62.04 (1.72\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op8}&\textbf{48.11 (7.05\%$\uparrow$)}  &   \textbf{91.36 (0.63\%$\uparrow$)} &  \textbf{62.66 (2.74\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op9}&\textbf{48.10 (7.03\%$\uparrow$)}   &   \textbf{91.50 (0.78\%$\uparrow$)} &  \textbf{62.70 (2.80\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op10}&44.91 (0.07\%$\downarrow$)   &   \textbf{90.86 (0.07\%$\uparrow$)} &  60.97 (0.03\%$\downarrow$)\\ \hline
\end{tabular}
\end{table}
\end{comment}

==> Testing Machine Learning based Code Generation Models/table/rq2_tab.tex <==
\begin{table}[]

\caption{ Performance of different operators on {\neuralCodeSum}, {\codeseq}, and {\codevec}. 
`Original' shows the \textit{1k original} test set.  
`Op1'--`Op10' represent the test sets with the perturbations introduced by one mutation operator respectively.  
Numbers in the brackets are the performance decline of the examined neural models on the mutated test set compared with the original test set.}
\label{tab:rq2_comp}

\begin{tabular}{clll}
\toprule \hline
\multicolumn{1}{c}{}    & \multicolumn{1}{c}{\textbf{\neuralCodeSum}} & \multicolumn{1}{c}{\textbf{\codeseq}} & \multicolumn{1}{c}{\textbf{\codevec}} \\ 
& \multicolumn{1}{c}{BLEU (\%)}   & \multicolumn{1}{c}{F1 (\%)} & \multicolumn{1}{c}{F1 (\%)}     \\ \hline
%\multicolumn{1}{l}{\bf Test data}  &&&\\%\cline{1-1}
\multicolumn{1}{l}{Original} & 40.82    &  71.16   &  47.68   \\\hline
\multicolumn{1}{l}{Op1}& 8.59 (78.95\%$\downarrow$)  &  68.23 (4.29\%$\downarrow$)  &  45.32 (5.05\%$\downarrow$) \\ 
\multicolumn{1}{l}{Op2}&  8.88 (78.26\%$\downarrow$)  &  70.75 (0.58\%$\downarrow$)   & 47.50 (0.23\%$\downarrow$)    \\ 
\multicolumn{1}{l}{Op3}&  8.84 (78.34\%$\downarrow$) &  70.70 (0.65\%$\downarrow$)   &    47.15 (0.97\%$\downarrow$) \\ 
\multicolumn{1}{l}{Op4}&  9.29 (77.21\%$\downarrow$)  & 70.85 (0.43\%$\downarrow$)    &   47.10 (1.08\%$\downarrow$)  \\ 
\multicolumn{1}{l}{Op5}&  \textbf{6.02 (85.25\%$\downarrow$)}  &  60.57 (17.49\%$\downarrow$)   &    44.73 (6.32\%$\downarrow$) \\ %\hline
\multicolumn{1}{l}{Op6}&  6.16 (84.90\%$\downarrow$) &   \textbf{58.65 (21.33\%$\downarrow$)}  &  44.78 (6.32\%$\downarrow$) \\ %\hline
\multicolumn{1}{l}{Op7}&  6.23 (84.73\%$\downarrow$)  &  59.82 (18.96\%$\downarrow$)   &    46.13 (3.21\%$\downarrow$)   \\ %\hline
\multicolumn{1}{l}{Op8}&  7.19 (82.38\%$\downarrow$)  &  64.67 (10.04\%$\downarrow$)  &  43.81 (8.69\%$\downarrow$)  \\ %\hline
\multicolumn{1}{l}{Op9}&  7.16  (82.45\%$\downarrow$) &  63.72 (11.68\%$\downarrow$)   & \textbf{41.04 (16.01\%$\downarrow$)}  \\ %\hline
\multicolumn{1}{l}{Op10} & 37.08  (9.16\%$\downarrow$)   &    71.06 (0.14\%$\downarrow$) &  47.49 (0.25\%$\downarrow$)   \\ 
\bottomrule \hline
\end{tabular}
\end{table}

%(Ori, 0.4761) (Op1, 0.4532) (Op2, 0.4759) (Op3,0.4715) (Op4, 0.4713) (Op5, 0.4473) (Op6, 0.4478) (Op7,0.4613) (Op8,0.4380) (Op9, 0.4104) (Op10, 0.4749);

==> Testing Machine Learning based Code Generation Models/table/rq3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering

\caption{Comparison results across original test sets, newly generated test sets using Random@3 and NC-guided ({\tool}) strategies. NC denotes Neuron Coverage and JD is the Jaccard Distance.}
\label{tab:rq3}
\setlength{\tabcolsep}{3pt}
\scalebox{0.9}{
\begin{tabular}{ccclcc}
\toprule \hline

\textbf{Model}   & \textbf{Strategies} & \textbf{\#New Tests} & \textbf{Performance (\%)} & \textbf{NC(\%)} &\textbf{JD} \\ \hline 
\multirow{3}{*}{\neuralCodeSum}     & \textit{1k original}    & -   &   BLEU = 40.82& 44.94 & - \\ %\cline{2-6} 
                                & Random@3      &  3,000  &  BLEU=8.59 (78.95\%$\downarrow$) &  47.39      &   0.29    \\ %\cline{2-6} 
                                & NC-guided     & 2,906   &   BLEU=6.20  (84.81\%$\downarrow$) &   48.95    &  0.32  \\ 
                             
                                \hline \hline
\multirow{3}{*}{\codeseq} & \textit{1k original}     & -   &   F1 = 71.16 & 90.79 &  - \\ %\cline{2-6} 
                            & Random@3      &  3,000  &  F1=63.36 (10.96\%$\downarrow$) & 95.15    & 0.05 \\ %\cline{2-6} 
                          & NC-guided     &  2,969  &  F1=55.46 (22.06\%$\downarrow$) & 95.71     & 0.08 \\ 
                          \hline \hline
\multirow{3}{*}{\codevec}  & \textit{1k original}     & -   &   F1 = 47.68 & 60.99    & - \\%\cline{2-6} 
                          & Random@3      &  3,000  &  F1=42.93 (9.96\%$\downarrow$)   & 72.24    &  0.17  \\ %\cline{2-6} 
                          & NC-guided     &  3,000  &   F1=34.53 (27.58\%$\downarrow$) & 75.23    & 0.25   \\  
                                        
                          \bottomrule \hline 
\end{tabular}
}
\end{table}

==> Testing Machine Learning based Code Generation Models/table/rq4.tex <==
\begin{table}[t!]
\centering
\setlength{\tabcolsep}{3pt}
\caption{ \small Model retrain scenarios and the corresponding performance. 
\textbf{TrData} indicates the randomly selected 10K training data from the original training dataset. 
%\textbf{`1k Or'} indicates the \textit{1k original} test data. 
%\textbf{`1k Or + 1k Mu'} indicates the \textit{1k original} test data and 1k mutants generated from it via randomly selected mutation operators.
\textbf{TrData+{\tool}} indicates an enhanced training dataset by combining \textbf{TrData} and the synthetic inputs generated by applying {\tool} on \textbf{TrData}.
\textbf{TrData+Random} indicates an enhanced training dataset by combining \textbf{TrData} and the synthetic inputs generated by applying \texttt{Random@3} on \textbf{TrData};}
\label{tab:rq4}
\scalebox{1}{
\begin{tabular}{lll}
\hline
\textbf{Model}     & \textbf{Training data} & \textbf{\textbf{Performance (\%)}} \\ \hline
\multirow{3}{*}{\neuralCodeSum} &TrData & BLEU = 16.50  \\ 
   &TrData+Random & BLEU = 20.32   \\ 
   &TrData+{\tool}&  \textbf{BLEU = 22.30}    \\ \hline  \hline
\multirow{3}{*}{\codeseq}       &TrData & F1 = 22.98  \\  
   &TrData+Random &   F1 = 23.16    \\ 
   &TrData+{\tool} &  \textbf{F1 = 25.01} \\  \hline  \hline
\multirow{3}{*}{\codevec}       &TrData & F1 = 11.54  \\ 
   &TrData+Random  &  F1 = 15.13  \\ 
   &TrData+{\tool}      &  \textbf{F1 = 15.48}   \\ \hline
\end{tabular}
}
\end{table}



==> figure/dis1.tex <==
\begin{figure}[t!]
\centering
\begin{subfigure}{0.5\textwidth}
\centering
\input{figure/discussion1.tex}
\end{subfigure}\hfill
\vspace{-0.1in}
\caption{\small 
The performance distribution of affected mutation operators.}
\vspace{-0.1in} 
\label{fig:dis1}
\end{figure}

==> figure/discussion2_1.tex <==
\begin{figure}[th!]
\centering
\footnotesize
%\begin{subfigure}{0.45\linewidth}
%\centering
 \scalebox{.5}{\input{figure/pie_1.tex}}
%\end{subfigure}
\caption{\small The distribution of selected mutation operators in {\neuralCodeSum} mutants dataset.}
\label{fig:dis_2_1}
\end{figure}


==> figure/discussion2_2.tex <==
\begin{figure}[th!]
\centering
\footnotesize
%\begin{subfigure}{0.45\linewidth}
%\centering
 \scalebox{.5}{\input{figure/pie_2.tex}}
%\end{subfigure}
\caption{\small The distribution of selected mutation operators  in {\codeseq} mutants dataset.}
\label{fig:dis_2_2}
\end{figure}


==> figure/discussion2_3.tex <==
\begin{figure}[th!]
\centering
\footnotesize
%\begin{subfigure}{0.45\linewidth}
%\centering
 \scalebox{.5}{\input{figure/pie_3.tex}}
%\end{subfigure}
\caption{\small The distribution of selected mutation operators  in {\codevec} mutants dataset.}
\label{fig:dis_2_3}
\end{figure}


==> figure/new_discussion2.tex <==
\begin{figure*}[t!]
\centering
\begin{subfigure}{0.32\linewidth}
\centering
 \scalebox{.6}{\input{figure/pie_1.tex}}
\caption{{\neuralCodeSum}}
\label{pie:d1}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
	\centering
 \scalebox{.6}{\input{figure/pie_2.tex}}
	\caption{{\codeseq}}
\label{pie:d2}
\end{subfigure}
\begin{subfigure}{0.32\linewidth}
	\centering
 \scalebox{.6}{\input{figure/pie_3.tex}}
	\caption{{\codevec}}
\label{pie:d3}
\end{subfigure}\hfill
\caption{ 
The distribution of selected mutation operators on the three models.}
\label{fig:new_dis_conbuild}
\end{figure*}

==> figure/pie_1.tex <==
\begin{tikzpicture}
\pie[text=pin, color ={black!3, black!10, black!20, black!30, black!40, black!50, 
black!55, black!60, black!65, black!70}]
{9.05/Op1, 8.39/Op2, 4.43/Op3, 
2.82/Op4, 15.79/Op5, 14.83/Op6,
13.97/Op7, 12.73/Op8, 
13.21/Op9, 4.74/Op10}
\end{tikzpicture}


==> figure/rq2_4_plot.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figure/NeuralCodeSum_rq2_4.png}
\caption{Difference in neuron coverage caused by different mutation operators in  {\neuralCodeSum}.}
\label{fig:rq2_4_plot}
\end{figure}

==> figure/rq2_5_plot.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figure/code2seq_rq2_5.png}
\caption{Difference in neuron coverage caused by different mutation operators in  {\codeseq}.}
\label{fig:rq2_5_plot}
\end{figure}

==> figure/rq2_6_plot.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figure/code2vec_rq2_6.png}
\caption{ Difference in neuron coverage caused by different mutation operators in {\codevec}.}
\label{fig:rq2_6_plot}
\end{figure}

==> sec/algorithm.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[t]
\caption{\small Coverage-Guided Test Generation in {\tool} \label{alg:algorithm0}}
\hrule
	\begin{algorithmic}[1]
		\small
		\vspace{.2cm}
		\REQUIRE %\scriptsize
		Seed programs \textit{S}, 
		Target neural model \textit{NM},\\
		Mutation function $mutate$; \\
		Mutation operators \textit{Ops}\\
		Neuron count cache $NCount$;\\
		Mutate operator set $MO;$ \\
		%Neural Activation function %$neuronActivation;$\\
		Maximum mutation \textit{MAX}; \\
	
		\ENSURE ~\\
		Generated tests $T$;
		\WHILE {$S$ is not empty}
		\STATE $p \longleftarrow S.pop() $
		\STATE $NC_p \longleftarrow neuronActivation(p, NM) $
        \STATE $mutry = 1$
		\WHILE {mutry $<=$ MAX}
		\STATE $mutry = mutry+1$
		\STATE $mutants \longleftarrow null $
		\STATE $bestIdx = -1 $
		\FOR   {$idx=0; idx<size(MO); idx++$} 
		\STATE $Mutant = mutate(O,p)$; 
		\STATE $Mutants.push(Mutant)$; 
		\STATE $NC_{mu}$ = $newNeuronActivation(Mutant,NC_p,NM)$
		\IF  { $size(NC_{mu})>size(NC_{p}) $}
		\STATE $bestIdx = idx$
		\ENDIF
		\ENDFOR
		\IF  { $bestIdx == -1 $}
		\STATE $break$
		\ENDIF
		\STATE $p=Mutants[bestIdx]$
		\STATE $NC_p = newNeuronActivation(p,NC_p,NM) \cup NC_p$
		\STATE T.push($p$) 
		\ENDWHILE
		\ENDWHILE
	\end{algorithmic}
	\hrule
\end{algorithm}


==> table/rq2_nc_2.tex <==
\begin{table}[t!]
\centering
\caption{Neuron coverage of different mutation operators. Values are in percentage. Numbers in the brackets are the number of new activated neurons.
\todo{Moshi:fill the number of new activated neurons }}%\jie{I seems that this figure is similar with Table IV. do we use the same format? XX (YY\% up or down?)}}
%\todo{moshi}}
\label{tab:rq2_nc_2}
\begin{tabular}{c|c|c|c|}
\cline{2-4}
   & \textbf{{\neuralCodeSum}} & \textbf{{\codeseq}} & \textbf{{\codevec}} \\ \hline
\multicolumn{1}{|l|}{Op1}&\textbf{722.80 }   &   \textbf{39.08}  &  \textbf{19.13 }\\ \hline
\multicolumn{1}{|l|}{Op2}&\textbf{702.65 }   &           16.72   &  \textbf{32.90 }\\ \hline
\multicolumn{1}{|l|}{Op3}&\textbf{702.32 }   &           11.17   &          25.12  \\ \hline
\multicolumn{1}{|l|}{Op4}&\textbf{700.31 }   &           19.80   &  \textbf{31    }\\ \hline
\multicolumn{1}{|l|}{Op5}&\textbf{745.05 }   &           55.83   &  \textbf{50.82 }\\ \hline
\multicolumn{1}{|l|}{Op6}&\textbf{742.95 }   &           55.44   &  \textbf{44.40 }\\ \hline
\multicolumn{1}{|l|}{Op7}&\textbf{741.40 }   &           53.99   &  \textbf{41.91 }\\ \hline
\multicolumn{1}{|l|}{Op8}&\textbf{768.31 }   &   \textbf{52.39 } &  \textbf{48.44 }\\ \hline
\multicolumn{1}{|l|}{Op9}&\textbf{772.08 }   &   \textbf{53.21 } &  \textbf{49.41 }\\ \hline
\multicolumn{1}{|l|}{Op10}&       459.86     &   \textbf{21.82 } &          25.17 \\ \hline
\end{tabular}
\end{table}








\begin{comment}
\begin{table}[t!]
\centering
\caption{Neuron coverage of different mutation operators. Values are in percentage. Numbers in the brackets are the difference.}%\jie{I seems that this figure is similar with Table IV. do we use the same format? XX (YY\% up or down?)}}
%\todo{moshi}}
\label{tab:rq2_nc}
\begin{tabular}{c|c|c|c|}
\cline{2-4}
   & \textbf{{\neuralCodeSum}} & \textbf{{\codeseq}} & \textbf{{\codevec}} \\ \hline
\multicolumn{1}{|l|}{Original} &44.94&   90.79 &  60.99\\ \hline
\multicolumn{1}{|l|}{Op1}&\textbf{47.33 (5.32\%$\uparrow$)} &\textbf{1.46 (0.74\%$\uparrow$)}&  \textbf{61.48 (0.80\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op2}&\textbf{47.07 (4.74\%$\uparrow$)}&   90.73 (0.06\%$\downarrow$) &  \textbf{61.00 (0.02\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op3}&\textbf{47.06 (4.72\%$\uparrow$)}&   90.76 (0.03\%$\downarrow$) &  60.98 (0.02\%$\downarrow$)\\ \hline
\multicolumn{1}{|l|}{Op4}&\textbf{45.75 (1.80\%$\uparrow$)}   &   90.68 (0.12\%$\downarrow$)&  \textbf{61.17 (0.29\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op5}&\textbf{47.55 (5.81\%$\uparrow$)}   &   88.61 (2.40\%$\downarrow$)&  \textbf{62.37 (2.26\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op6}&\textbf{47.49 (5.67\%$\uparrow$)}   &   89.53 (1.38\%$\downarrow$) &  \textbf{62.33 (2.19\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op7}&\textbf{47.48 (5.65\%$\uparrow$)}   &   88.98 (1.99\%$\downarrow$) &  \textbf{62.04 (1.72\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op8}&\textbf{48.11 (7.05\%$\uparrow$)}  &   \textbf{91.36 (0.63\%$\uparrow$)} &  \textbf{62.66 (2.74\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op9}&\textbf{48.10 (7.03\%$\uparrow$)}   &   \textbf{91.50 (0.78\%$\uparrow$)} &  \textbf{62.70 (2.80\%$\uparrow$)}\\ \hline
\multicolumn{1}{|l|}{Op10}&44.91 (0.07\%$\downarrow$)   &   \textbf{90.86 (0.07\%$\uparrow$)} &  60.97 (0.03\%$\downarrow$)\\ \hline
\end{tabular}
\end{table}
\end{comment}
